A Theory of Formal Synthesis via Inductive Learning

Formal synthesis is the process of generating a program satisfying a high-level formal specification. In recent times, effective formal synthesis methods have been proposed based on the use of inductive learning. We refer to this class of methods that learn programs from examples as formal inductive synthesis. In this paper, we present a theoretical framework for formal inductive synthesis. We discuss how formal inductive synthesis differs from traditional machine learning. We then describe oracle-guided inductive synthesis (OGIS), a framework that captures a family of synthesizers that operate by iteratively querying an oracle. An instance of OGIS that has had much practical impact is counterexample-guided inductive synthesis (CEGIS). We present a theoretical characterization of CEGIS for learning any program that computes a recursive language. In particular, we analyze the relative power of CEGIS variants where the types of counterexamples generated by the oracle varies. We also consider the impact of bounded versus unbounded memory available to the learning algorithm. In the special case where the universe of candidate programs is finite, we relate the speed of convergence to the notion of teaching dimension studied in machine learning theory. Altogether, the results of the paper take a first step towards a theoretical foundation for the emerging field of formal inductive synthesis.

==> intro-old.tex <==

\section{Introduction}\label{sec-intro}

There has been enormous advances in automated formal methods in recent years. 
Formal techniques such as model checking~\cite{clarke-mc} and theorem proving~\cite{clark-smt}
have acheived impressive scalability and are routinely used in industry for
computer-aided design of integrated circuits~\cite{fix-formal,seger-fm,ganesh-fm}, 
finding bugs in software~\cite{woodcock-fm,Emanuelsson-sa} and model-based
design of cyberphysical systems~\cite{simulink,labview}. Synthesis is often
used in generating verification artifacts such as loop invariants in 
program verification~\cite{sankaranarayanan2004non,wegbreit1974synthesis},
pre and post conditions for functions~\cite{bjorner2014applications}, 
environment assumptions~\cite{li2011mining}, 
ranking functions~\cite{podelski2004complete}, control invariants~\cite{sankaranarayanan2004constructing}
as well as abstraction and refinement in model checking~\cite{clarke-cegar}.
Use of these verification artifacts has been the key to enable composable and modular verification
which can scale easily to large industrial systems. 
Synthesis also 
enables generation of verification collaterals such as mining of specification for verification
and modeling environment assumptions. A detailed discussion of interplay between formal verification and synthesis
has been previously surveyed~\cite{seshia-dac12}.
Beyond its utility in generating formal verification collaterals and artifacts, 
automatic synthesis of systems from high-level specifications
has also been a long-standing goal 
of the fields of electrical engineering and computer science.  
Recently, the massive improvement in scalability of theorem proving techniques
has led to resurgence of interest in automated synthesis of systems, particularly programs~\cite{alur-fmcad13}.
These techniques employ a diverse set of  techniques 
and are targetted towards a large spectrum of applications.
Despite their apparent heterogenity, 
they share a common methedology of merging deductive formal verification techniques
with inductive generalization from examples.
In this paper, we make an attempt to factor out this common paradigm and call it
{\it {formal methods}}. We identify and discuss some important theoretical questions about this
paradigm which enables comparison of different techniques implementing this paradigm. 
While the target of synthesis techniques can be various different artifacts, we focus on
synthesis of programs as many of these artifacts which have discrete input and output can be 
described as programs.

Automatic synthesis of programs has found many practical
applications such as generating optimal code sequences~\cite{Massalin87,Joshi02},
optimizing performance-critical inner loops, generating
general-purpose peephole optimizers~\cite{Bansal06,bansal08},
automating repetitive programming,
and filling in low-level
details after the higher-level intent has been expressed~\cite{asplos06}
as well as symbolic planning over discrete domain in robotics~\cite{nedunuri-plan}.
A traditional view of program synthesis is that of synthesis
from complete specifications. One approach is to give
a specification as a formula in a suitable logic~\cite{Manna80,Manna92fundamentalsof,jha-11}.
Another is to write the specification as a simpler, but
possibly far less efficient program~\cite{Massalin87, asplos06,Joshi02}.
All these different variants
of automated synthesis techniques share some common characteristics. They
are iterative inductive synthesis techniques which require some kind of validation
engines to validate candidate programs produced at intermediate iterations, and
these validation engines identify
counterexamples, aka mistakes, which are subsequently used for inductive synthesis in the next iteration.
We collectively refer to such synthesis techniques as
counterexample-guided inductive synthesis, aka $\tcegis$.
While these
approaches have the advantage of completeness of specification,
such specifications are often unavailable, difficult to
write, or expensive to check against using automated verification
techniques. This has led to proposal of alternative synthesis approach~\cite{jha-icse10}
in which the complete specification is not available and distinguishing inputs 
are used to generate interesting examples for induction. Stochastic sampling of inputs~\cite{Schkufza-stochastic}
and arbitrary enumeration~\cite{Udupa-snippet} have also being proposed as alternative methods of generating
examples for synthesis. A detailed study of these synthesis approaches and a common framework of 
syntax guided synthesis has been previously proposed in literature to present a unified definition
of synthesis problem~\cite{alur-fmcad13}.
The input to the syntax-guided synthesis problem (SyGuS)~\cite{alur-fmcad13} consists of a background theory, 
a semantic correctness specification for the desired program given by a logical formula, 
and a syntactic set of candidate implementations given by a grammar. 
The computational problem then is to find an implementation from the set of candidate expressions so that 
it satisfies the specification in the given theory. 
While SyGuS defines a generic architecture for synthesis ~\cite{alur-fmcad13} which use
verification to identify the correct program, our goal is to focus on identifying key components of
formal synthesis approaches and to present a therotical analysis based on varying properties of these components.
SyGus defines a class of synthesis problems
that could be solved either using learning (inductive
synthesis) or purely deductively. We attempt to define a unified solution paradigm of synthesis which presents
one approach to solve SyGus problems as well as other synthesis problems. 

Automated synthesis from examples has been well studied in artificial intelligence~\cite{Russell-ai}
and machine learning~\cite{Mitchell-ml}.
The targets of such synthesis approaches are often concepts such as linear or polynomial equations~\cite{regression}, 
convex polytopes~\cite{Hegedus-convex},
Boolean formulae~\cite{Jackson-dnf} and decisions trees~\cite{Quinlan-decisiontrees}.
Concepts in automated synthesis in machine learning is analogous to programs in synthesis using formal methods. 
Statistical and algorithmic learning techniques have been proposed to address this problem. While
statistical techniques~\cite{hastie01statisticallearning}
can identify concepts in presence of noise and often scale well for simple
concepts over inputs that come from independent and identical distributions (i.i.d) of point samples, 
these techniques are not well suited for learning
complex concepts or for learning with structured data such as relations. They also do usually
not provide hard correctness guarantees 
on the learned concept. There has been significant work on learning of concepts from examples in
the field of algorithmic learning~\cite{gold67limit}
but most of the work is theoretical. Unlike statistical learning approaches,
algorithmic learning does not assume that the input data comes from a random distribution and is independent
of each other. This makes it more suited for learning languages~\cite{gold67limit} 
and automata~\cite{angluin88}. Formal synthesis differs from identification of concepts in machine
learning across three dimensions.
\begin{itemize}
\item Inductive engines used for generalization:
Formal synthesis uses general-purpose decision procedures and model checkers rather than custom learning algorithms.
\item Oracle providing examples:
Formal synthesis involves active learning in presence of an oracle 
(which could be a human user or another decision procedure) which could provide responses to a rich set
of queries. This is in contrast to batch learning or active learning
from oracles which only select examples from a large corpus and do not make richer queries. Also, the examples
are not assumed to be indepenent of each other or coming from a particular random distribution.
\item Guarantees on the synthesis: Formal synthesis has emphasis on exact learning. If the exact concept cannot
be inferred, then the formal synthesis approach should report failure rather than identifying the closest 
possible concept.
\end{itemize}


We present a formal synthesis paradigm which combines the ideas from formal methods and algorithmic learning.
Formal synthesis can be described as an interaction between the two key 
components: an induction engine which queries an oracle and generalizes from response of the queries to propose
hypothesis programs or concepts, and an oracle which provides response to queries from the induction engine.
We call this formal synthesis paradigm as 
{\it { Oracle-Guided Inductive Synthesis} }, aka, $\ogis$. 
%Figure~\ref{label:ogis} illustrates the $\ogis$ paradigm.
The different $\ogis$ techniques differ from each other in two important ways:
\begin{itemize}
\item the types of queries supported by Oracle: For example, Oracle could provide only positive examples, or
provide positive examples as well as negative examples which refute proposed hypothesis programs generated
by induction engine. Oracle could also support queries which request particular kind of counterexamples such as 
minimal counterexamples.
\item the generalization approach used by the induction engine: For example, the induction
engine could be assumed to have a finite memory or infinite unbounded memory. One could
also use computational complexity of the induction algorithm to differentiate synthesis techniques.
\end{itemize}

In this paper, we conduct a theoretical study of $\ogis$  by examining the impact
of using different kinds of queries, and considering induction engines with finite and infinite memory.
Inferring programs from a finite class iteratively using queries can be easily shown to terminate for queries
which ensure progress, for example, queries that provide a new example in every iteration.
But termination is not guaranteed for programs which do not belong to a finite class.
Most of the existing synthesis techniques are applied to problems with the assumption that the number
of examples, both positive and negative, is finite and consequently the programs that can be synthesized
is also finite. But even in practical applications such as programs over finite precision data variables
and hardware circuits, the set of examples, say input/output samples is finite but it is often too large.
Also, design of algorithms, controllers, control invariants and plans require reasoning with infinite
data types. The synthesis power of $\ogis$ techniques is determined by the class of programs that can 
be synthesized successfully from examples by the technique.
We investigate how using different kinds of queries in $\ogis$ change the synthesis power
of $\ogis$ techniques. We also examine how restricting the generalization approach to use only finite
memory effects the synthesis power of $\ogis$ techniques. 
We make the following contributions in the paper:
\begin{itemize}
\item We propose a formal synthesis paradigm: {\it {Oracle-Guided Inductive Synthesis} } ($\ogis$) and illustrate
how it generalizes instances of concept learning in machine learning/artificial intelligence as well as 
synthesis techniques developed using formal methods. We provide examples of synthesis techniques from literature
and show 
\item We use the $\ogis$ paradigm to develop a theoretical framework to compare synthesis techniques in terms
of their synthesis power. The synthesis power is defined using the class of programs that can be synthesized
using the synthesis technique. We
establish the following novel theoretical results:
\begin{itemize}
\item For inductive engines that can use unbounded memory, the power of synthesis engines using oracle 
that provides arbitrary counterexamples or minimal counterexamples is the same. But this is strictly more 
powerful than using oracle which provides counterexamples which are bounded by
the size of the positive examples.
\item For inductive engines that use bounded memory, the power of synthesis engines using arbitrary counterexamples
or minimal counterexamples is still the same. 
%The oracle providing counterexampels by a constant is stricly less powerful but 
The power of synthesis engines using counterexamples bounded by positive examples is not comparable
to those using arbitrary/minimal counterexamples. Contrary to intuition, using counterexamples bounded by positive
examples allows one to synthesize programs from program classes which cannot be synthesized using arbitrary or
minimal counterexamples.
\end{itemize}
\end{itemize}

The rest of the paper is organized as follows.
We first present the 
{\it {Oracle Guided Inductive Synthesis}} ($\ogis$) paradigm in
Section~\ref{sec-ogis}. We discuss related work in Section~\ref{sec-rel}. We present the notation
and definitions used for theoretical analysis in Section~\ref{sec-not} followed by the theoretical
results and their proofs in Section~\ref{sec-res} and Section~\ref{sec-finres}. 
We discuss open problems and conclude in
Section~\ref{sec-con}.



==> notation.tex <==

\section{Preliminaries} \label{sec-not}


Our presentation of formal inductive synthesis and \ogis so far has
not used a particular representation of a concept class or
specification. In order to prove our theoretical results, such a
choice is necessary. In this section, we precisely define the formal
inductive synthesis problem for concepts (programs) that correspond to
recursive languages. We restrict our attention to the case when the
specification is complete and is defined by such a language. 
We give precise definitions of the variants of CEGIS under study in
the rest of the paper. 
For ease of reference, the major definitions and frequently
used notation are summarized 
in Table ~\ref{table:not}.

\subsection{Notation}

We describe here the notation used in the paper. $\nat$ represents  the set of natural numbers. 
$\nat_i \subset \nat$ denotes a subset of natural numbers $\nat_i = \{ n | n < i\}$. 
Consider a set $S \subset \nat$. $\min(S)$ denotes the minimal element in $S$. 
The union of the sets is denoted by $\cup$ and the intersection of the sets
is denoted by $\cap$. $S_1\setminus S_2$ denotes set minus operation with the resultant set containing
all elements in $S_1$ and not in $S_2$.

\todo{
A sequence $\sigma$ is a mapping from $\nat$ to $\nat \cup \{\bot\}$.
We denote a prefix of length $k$ of a sequence by $\sigma[k]$.
So, $\sigma[k]$ of length $k$ is a mapping from $\nat_k$ to $\nat \cup \{\bot\}$ for $k \leq i$.
}
$\sigma[0]$ is an empty sequence also denoted by $\sigma_0$ for brevity. 
We denote the natural numbers in the range of $\sigma[i]$ by $\samples$, 
that is, $\samples(\sigma_i) = \range(\sigma_i) - \{\bot\}$.
The set of sequences is denoted by $\Sigma$.

%We extend natural numbers to pairs. Let $\langle n_1, n_2 \rangle$ be any
%bijective computable function from $\nat \times \nat \rightarrow \nat$
%which is monotonically increasing in both of its arguments. Similarly, pairs
%can be extended to $n$-tuples. Assuming existence of such a bijective mapping,
%tuples can also be used in place of natural numbers as elements of a language.
%A language in this case would be a subset of such tuples.

We also use standard definitions from computability theory~\cite{rogers-book87}. A set $\lang_i$ of 
natural numbers is called computable or recursive  language if there is a program, that is, a 
computable, total function $\algo_i$ such that for any natural number $n$, 
$$\algo_i(n) = 1 \; \mathtt{ if } \;  n \in \lang_i \; \mathtt{ and } \; \algo_i(n) = 0 \; 
\mathtt{ if } \; n \not \in \lang_i$$
We say that $\algo_i$ {\em identifies} the language $\lang_i$.
\st{
We denote the complement of language $\lang_i$ by $\overline \lang_i = \nat \setminus \lang_i$. 
We denote the union of two languages $L_i$ and $L_j$ by $L_i \cup L_j$, 
and the intersection of two languages $L_i$ and $L_j$ by $L_i \cap L_j$.
} 
Also for convenience, we use $\langfun(\algo_i)$ to denote $\lang_i$ using the mapping between 
languages and programs that identify them. Thus, we distinguish only between semantically different
programs and not the syntactically different programs which identify the same language. Recall that
there is a program that identifies a language if and only if it is a recursive language. In this 
paper, we restrict our discussion to recursive languages 
because it includes many interesting and natural classes of languages
that correspond to programs and functions of various kinds, including regular, context free, context
sensitive, and pattern languages.
%constitute indexable classes of recursive languages.

Given a sequence of non-empty languages 
$ \mathscr{\lang} = \lang_0, \lang_1, \lang_2, \ldots$, $\mathscr{\lang}$ is said to be an indexed family of languages 
if and only if there exists a recursive function $\template$ such that $\template(i,n) = \algo_i(n)$. 
We denote the corresponding set of programs $\algo_0, \algo_1, \algo_2, \ldots$ by $\mathscr{\algo}$. 
For brevity, we refer to $\template(i,n)$ also as $\algo_i(n)$. Intuitively,
$\template$ defines the encoding of candidate program space similar
to sketches in $\cite{asplos06}$ and the component interconnection encoding in
$\cite{jha-icse10}$. The index $i$ is used to index into this encoding to select a particular
program $\algo_i$. $\algo_i(n)$ denotes the output of the program on input $n$. $\algo_i(n) = 1$
if and only $n \in \lang_i$, and $\algo_i(n) = 0$ otherwise. In
practice, we often consider a family of candidate programs in synthesis
which contain syntactically
different programs which are semantically equivalent, that is,
there are syntactically different 
programs which have the same set of behaviors. 
Thus, templates in synthesis may allow a choice in picking $j$ such 
that $\template(j,n) = P_i(n)$ for $j \in J_i$ where the set $J_i$ 
represents syntactically different but semantically equivalent programs
that produce output $1$ on an input if and only if the
input natural number belongs to $\lang_i$.
Our approach relies on finding the subset of behaviors represented
by natural numbers which unqiuely identify the correct behavior set,
represented by $\lang_i$, of the target program 
and thus, synthesis corresponds to identifying a semantically
correct program. If there are semantic clones, identifying any one 
of them would be sufficient. 
So, we consider $\template(i,n)$ to be the set of semantically 
different programs such that the program $\algo_i$ corresponds to 
the set of behaviors in language $\lang_i$.


\todo{
The languages are isomorphic to sets of natural numbers. 
The ordering of natural numbers can be used
to order members of a language so that $\min(\lang)$ denotes the minimal member of the language
$\lang$. In practice, languages corresponding to a program are sets of
input/output traces of
the program\footnote{Note that the encoding to natural numbers means that we restrict our attention to
programs whose traces are finite-length or, more generally, finitely representable}. 
We can construct a totally ordered set of all possible input/output traces 
using any ordering such as a lexicographic ordering over a trace sequence
combined with a total ordering over elemens of the sequence.
We can then map the traces to the set of natural numbers using this ordering.
}
%This set is isomorphic to the set of natural numbers $\nat$.
%Any ordering of the set elements can be chosen; for example, strings could be ordered
%lexicographically. 
The choice of ordering is orthogonal to results presented in our paper. 
The natural number index of the trace in this ordered set of all traces 
can be used to represent it. 
So, our formulation of defining languages as subsets of $\nat$ and using the ordering 
over natural numbers is only a choice of convenience and does not restrict the generality of our results.


%Inductive synthesis consists of synthesis engines $\engine$ each of which identify the correct 
%program $\algo_i$ using a set of examples from the target language $\lang_i$ from a given indexed 
%family of languages $\mathscr{\lang}$. So, the overall synthesis problem is as follows.

\todo{
Let $\mathscr{\algo} = \{\algo_1, \algo_2, \ldots \} $ 
be the class of candidate programs corresponding
to an indexed family of languages~\cite{jain1999systems} 
$\mathscr{\lang} = \{\lang_1, \lang_2, \ldots \}$
such that $P_i$ identifies the language $L_i$, that is,
 $\algo_i(n) = 1 \; \mathtt{ if } \;  n \in \lang_i \; \mathtt{ and } \; \algo_i(n) = 0 \; 
\mathtt{ if } \; n \not \in \lang_i$.
}
 $\mathscr{\algo}$ defines a concept class $\class$ for synthesis.
The domain $\domain$ for synthesis is the set of natural numbers $\nat$
and the examples are $i \in \nat$.
The specification $\Spec$ correspond to the languages $\lang$ identified by 
programs. So, the formal inductive synthesis problem defined
in Section~\ref{sec-ogis} can be described
as follows for program synthesis using 
our notation:
\begin{definition}
Given a program class $\mathscr{\algo}$ over the domain of natural numbers
$\nat$, the formal inductive program synthesis problem is to find, using
$k$ oracles $\oracle_i: \mathscr{\algo} \rightarrow \nat, i = 1,\ldots, k$ and
a learning engine $\engine: (\nat^k)^* \rightarrow \mathscr{\algo}$,
a {\em target program} $\algo_{target} \in \mathscr{\algo}$ such that
$\algo_{target}$ identifies the target language $\lang_{target}$.
\end{definition}

As explained earlier, a common implementation of an oracle could be
a verifier which produces counterexamples or a sampling engine which
generates positive examples.

\comment{
Now, given some target language $\lang_i$ from a given indexed family of languages 
$\mathscr{\lang}$, the goal of inductive
synthesis is to synthesize the program $\algo_i$ from the candidate program space  $\mathscr{\algo}$
where $\algo_i$ corresponds to the language $\lang_i$. 
}


 
\begin{table}[h!]
\centering
\begin{tabular}{|c | c || c | c|} 
 \hline
 Symbol & Meaning & Symbol & Meaning \\ 
 \hline
 $\nat$ & natural numbers  & $\nat_i$ & natural numbers less than $i$\\ 
 $\min(S)$ & minimal element in set $S$ & $S_1 \setminus S_2$ & set minus \\
 $S_1 \cap S_2$ & set intersection & $S_1 \cup S_2$ & set union \\
 $\lang_i$ & language (a subset of $\nat$) & $\overline \lang_i$ & complement of language\\
 $\sigma$ & sequence of numbers & $\sigma_0$ & empty sequence \\
 $\algo_i$ & program for $\lang_i$ & $\langfun(\algo_i) = \lang_i$ & language corresponding to $\algo_i$\\
 $\samples(\sigma)$ & natural numbers in $\sigma$ & $\Sigma$ & set of language transcripts\\
 $\mathscr{\lang}$  & family of languages &  $\mathscr{\algo}$ & family of programs \\
\hline
 $\trace$ & transcript of language & $\ce$ & counterexample transcript\\
 $\engine$ & synthesis engine & $\learner$ & inductive learning engine\\
 $\verifier_\lang$ & verification oracle for language $\lang$ & $\mnverifier_\lang$ &  minimal counterexample $\verifier_\lang$\\
 $\bverifier_\lang$ & bounded counterexample $\verifier_\lang$ & $\hmnverifier_\lang$ & positive bounded counterexample $\verifier_\lang$ \\
 $\infcegis$ & \pbox{20cm} {language identified by\\ inf memory cegis engine} & $\cegis$ & \pbox{20cm}{language identified by\\  finite memory cegis engine}\\
 $\infmncegis$ & $\infcegis$ with $\mnverifier$ & $\mncegis$ & $\cegis$ with $\mnverifier$\\
 $\infbcegis$ & $\infcegis$ with $\bverifier$ & $\bcegis$ & $\cegis$ with $\bverifier$\\
 $\infhmncegis$ & $\infcegis$ with $\hmnverifier$ & $\hmncegis$ & $\cegis$ with $\hmnverifier$\\
\hline
\end{tabular}
\caption{Frequently used notation in the paper}
\label{table:not}
\end{table}


\comment{
The synthesis engine $\engine$ receives examples which belong to the language or are counterexamples
to previous hypothesis programs proposed by the engine. From these examples,
the synthesis engine $\engine$ needs to identify the correct program $\algo_i$.
}


\comment{

\textbf{TODO: below will probably migrate upwards from notation} 
We define inductive synthesis more formally in the next section. But intuitively, every inductive
synthesis consists of two steps:
\begin{itemize}
\item Inductive Generalization: This step generalizes from the presented examples to propose 
a hypothesis program from the candidate space of programs as the synthesized program.
\item Deductive Verification: This step validates the proposed hypothesis program and either
provides an example that invalidates the hypothesis program or it reports that it cannot find
such an example. 
\end{itemize} 

The soundness and completeness of the inductive synthesis techniques depend on the soundness
and completeness of both of these steps: inductive learning and deductive verification. 
Different inductive synthesis techniques differ from each other in their choice of how these two
steps are implemented. We identify two dimensions across which we can categorize the inductive
synthesis techniques:
\begin{itemize}
\item Memory: We consider inductive synthesis techniques which are restricted to use bounded finite memory,
as well as techniques which do not have any memory bounds. 
\textbf{TODO: mention here that the usual CEGIS etc falls under techniques which assume no memory bounds}
\item Deduction: We consider three possible different deductive techniques which can be used in synthesis.
The first deductive verification provides any arbitary counterexamples, the second provides 
counterexamples which are minimal and the third is restricted to providing counterexamples which are 
smaller than the largest example seen so far by the synthesis engine. 
\end{itemize}

\textbf{TODO: Switch away from cegis to inductive synthesis lest people digress and say this is not cegis etc
in rest of the paper too.
TODO: All discussions below on finite memory synthesis engine: rename and add material for inf memory}

%\section{Definitions}
 }

\subsection{Definitions}

We now present some key definitions used in rest of the paper.
\todo{Formal synthesis problem ($\synth$) has been previously 
defined in Section~\ref{sec-ogis}.}
\comment{
We begin by defining formal synthesis ($\synth$). It 
consists of inductive learning engine $\learner$ that learns using 
various kind of queries $\query_1, \ldots, \query_k$,
and an oracle $\oracle$ which provides responses
$\resp_1,  \ldots, \resp_k$ to these queries.
We use ${\overline {\query_j}}$ and ${\overline {\resp_j}}$ 
to denote sequences of
queries and responses of kind $j$ respectively, and
${\overline \query_j(i)}$ and ${\overline \resp_j(i)}$ denotes the $i$-th
query and response respectively in the sequence.

\begin{definition}
A formal synthesis engine $\engine_\ogis$ is
$$\engine_\ogis := \learner ({\overline \resp_1}, \ldots, {\overline \resp_k}) $$
where $\oracle({\overline \query_j(i)}) = {\overline \resp_j(i)}$.
\end{definition}
}
% Trace is a finite sequence of examples from the target language 
%$\lang$. The formal definition of trace is as follows:
Formal synthesis ($\synth$) techniques often employ 
%two kinds of oracles:
%a positive example generating oracle that can provide examples from the 
%target language, and
a verification engine 
%that can be used 
as an oracle which provides counterexamples.
We define the transcript sequence of positive examples and 
verifiers for a language formally below and then, 
\todo{give a formal 
definition of different
$\synth$ engines such as $\engine_{\cegis}$ which use these verifiers as oracle.} 
These verifiers correspond to the subsumption query discussed in 
Section~\ref{sec-ogis}. 
\todo{Counterexamples are generated by checking
the candidate language against the target language.}
Intuitively, the verifier returns a counterexample if it can
find an example that invalidates the proposed program, and 
returns $\bot$ otherwise.  



\begin{definition}
 { \todo{Transcript}} $\trace$: 
A \todo{transcript} $\trace$ for a language $\lang$ is a sequence with
 $\samples(\trace) = \lang$. $\trace[i]$ denotes the prefix of the \todo{transcript} $\trace$ of length $i$.
 $\trace(i)$ denotes the $i$-th element of the \todo{transcript}.
\end{definition}


\begin{definition}
A {verifier} $\verifier_\lang$ for a language $\lang$ is a non-deterministic mapping from 
$\mathscr{\lang}$ to $\nat \cup \{\bot\}$ such that $\verifier_\lang(\lang_i) = \bot$ if and only if
$\lang_i \subseteq \lang$, and $\verifier_\lang(\lang_i)  \in \lang_i \cap \overline \lang$ otherwise.
\end{definition}

We consider three other variants of verification oracle which generates particular nature of 
counterexamples instead of arbitrary counterexamples.
We define a minimal counterexample generating verifier. The counterexamples are minimal with respect
to an ordering of members in the language. In practice, if traces are used as examples, then a
minimal counterexample can be a trace of minimal length. 

\begin{definition}
A  {verifier} $\mnverifier_\lang$ for a language $\lang$ is a mapping from $\mathscr{\lang}$ to $\nat \cup \bot$ such that\\ $\mnverifier_\lang(\lang_i) = \bot$ if and only if $\lang_i \subseteq \lang$, and
$\mnverifier_\lang(\lang_i) = \min( \overline \lang \cap \lang_i)$ otherwise.
\end{definition}

Next, we consider another variant of counterexamples, 
namely (constant) bounded counterexamples. 
Bounded model-checking~\cite{biere-bmc} returns a counterexample trace for an incorrect design if it can find 
a counterexample of length less than the specified constant
bound. It fails to find a counterexample for an incorrect design
if no counterexample exists with length less than the given bound.
Verification of concurrent programs by bounding the number of context switches~\cite{qadeer-bounded} 
is another example of bounded verification technique. This motivates
the definition of a verifier which returns counterexamples bounded by a constant $\bound$.

\begin{definition}
A  {verifier} $\bverifier_{\lang,\bound}$ for a language $\lang$ is a mapping from 
\st{$\mathscr{\lang} \times \Sigma $} 
\todo{$\mathscr{\lang}$}
to $\nat \cup \bot$ such that\\ 
$\bverifier_{\lang,\bound}(\lang_i) = m$ where $m \in \overline \lang \cap \lang_i \wedge m < \bound$ 
for the given bound $\bound$, and $\bverifier_{\lang,\bound}(\lang_i,\trace[n]) = \bot$ otherwise.
\end{definition}

The last variant of counterexamples is  {\it positive bounded} counterexamples.
The verifier for generating positive bounded counterexample is also provided
with the \todo{transcript} seen so far by the synthesis engine. The verifier generates a counterexample
smaller than the largest positive example in the \todo{transcript}. If there is no counterexample smaller than the
largest positive example in the \todo{transcript}, then the verifier does not return any counterexample.
This is motivated by the practice of mutating correct traces to find bugs in programs and designs.
The counterexamples in these techniques are bounded by the size of positive examples (traces) 
seen so far.
 
\begin{definition}
A  {verifier} $\hmnverifier_\lang$ for a language $\lang$ is a mapping from $\mathscr{\lang} \times \Sigma $ to $\nat \cup \bot$ such that\\ $\hmnverifier_\lang(\lang_i,\trace[n]) = m$ where $m \in \overline \lang \cap \lang_i \wedge m < \trace(j)$ for some $j \leq n$, and $\hmnverifier_\lang(\lang_i,\trace[n]) = \bot$ otherwise.
\end{definition}

The synthesis engine using infinite memory can now be defined as follows.
\begin{definition}
An infinite memory 
$\infcegis$ engine $\engine_{\infcegis} : \Sigma \times \Sigma \rightarrow \mathscr{\algo}$ is 
a mapping 
$$\engine_{\infcegis} (\trace[n], \ce[n]) = \inflearner(\trace[n],\ce[n])$$ where
$\inflearner$ is a function 
$\Sigma \times \Sigma \rightarrow \mathscr{\algo}$ 
that characterizes the learning engine and how it eliminates counterexamples.
$\inflearner$ has infinite memory and can store unbounded
transcripts $\trace[n]$
and $\ce[n]$.
$\trace$ is a transcript for language 
$\lang$ and $\ce$ is a counterexample sequence such that
$$\ce(i) = \verifier_\lang(\langfun(\engine_{\infcegis}(\trace[i-1], \ce[i-1]))) $$
$\engine_{\infcegis} (\sigma_0, \sigma_0)$ is a predefined constant representing an initial guess 
$\algo_0$ of the program, which for example, could be program corresponding to the universal language $\nat$.
\end{definition}

If the oracles are not consistent and the same example is provided as 
a positive example as well as a counterexample, then the learning
engine cannot find any consistent program and it returns the program
corresponding to empty language. The counterexample to empty language by
the subsumption query verifier is $\bot$. So, the overall synthesis engine
produces the program corresponding to empty language $\emptyset$ when
it is not possible to synthesize a program consistent with the output of
oracles.

A synthesis engine with finite memory cannot store unbounded infinite 
transcripts. 
So, the $\cegis$ synthesis engine 
$\engine_{\cegis}$ maintains its current hypothesis program and some bounded memory at every iteration. 
An inductive learning function $\learner$ uses bounded memory and 
takes the current hypothesis program, an example
and a counterexample, and produces the corresponding next hypothesis program. 
$\learner$ can access 
additional state $\scratch$ stored by the synthesis engine in the finite bounded memory.

\begin{definition}
A finite memory 
$\cegis$ engine $\engine_{\cegis} : \Sigma \times \Sigma \rightarrow \mathscr{\algo}$ is defined recursively 
below.
$$\engine_{\cegis} (\trace[n], \ce[n]) = \learner( \engine_{\cegis} (\trace[n-1], \ce[n-1]),  \trace(n), \ce(n) , \scratch) $$
where $\learner$ is a recursive function 
$\mathscr{\algo} \times (\nat \cup \{\bot\}) \times (\nat \cup \{\bot\})  \times \Scratch \rightarrow \mathscr{\algo}$ 
that characterizes the learning engine and how it eliminates counterexamples,
$\scratch \in \Scratch$ is a finite state that might be maintained by the
learner beyond maintaining the current hypothesis, $\trace[n]$ is a 
transcript for language 
$\lang$ and $\ce$ is a counterexample sequence such that
$$\ce(i) = \verifier_\lang(\langfun(\engine_{\cegis}(\trace[i-1], \ce[i-1]))) $$
$\engine_{\cegis} (\sigma_0, \sigma_0)$ is a predefined constant representing an initial guess 
$\algo_0$ of the program, which for example, could be program corresponding to the universal language $\nat$.
\end{definition}

Intuitively, $\cegis$ is provided with a transcript along with a counterexample
transcript formed by counterexamples to the latest conjectured languages from the verifier $\verifier_\lang$.

\begin{definition}
We say that $\engine_{\cegis}$ converges to $\algo_i$, written 
$\engine_{\cegis}(\trace, \ce) \rightarrow \algo_i$, if and only if
there exists $k$ such that for all $n\geq k$, 
$$\engine_{\cegis}(\trace[n], \ce[n]) = \engine_{\cegis}(\trace[k], \ce[k]) = \algo_i$$
\end{definition}

\todo{
\begin{definition}
$\engine_{\cegis}$ identifies a language $\lang_i$ if and only if for any finite prefix transcript $\trace[n]$ such that
$\samples(\trace[n]) \subseteq \lang_i$, and counterexample sequences $\ce[n]$, the synthesis engine
converges to the language $\lang_i$
for some extension of the finite transcript, that is,
for some extension $\trace' \supseteq \trace[n]$ 
and $\ce \supseteq \ce[n]$, 
$\engine_{\cegis}(\trace', \ce) \rightarrow \algo_i$.
\end{definition}
}

\begin{definition}
$\engine_{\cegis}$ identifies a language family $\mathscr{\lang}$ if and only if 
$\engine_{\cegis}$ identifies every $\lang_i \in \mathscr{\lang}$.
\end{definition}

We now define the set of language families that can be identified by the 
inductive synthesis engines as $\cegis$ formally below.

\begin{definition}
$\cegis = \{ \; \mathcal{L} \; | \; \exists \engine_{\cegis} \; .\; \engine_{\cegis}$ identifies $\mathscr{\lang} \}$
\end{definition}

The convergence of synthesis engine to the correct language, 
identification condition for a language, and 
language family identified by a synthesis engine
are defined similarly in the case where the learning engine $\learner$
has infinite memory. 
The languages identified by the infinite memory synthesis engine 
$\engine_{\infcegis}$ is denoted by $\infcegis$.

We denote the infinite memory synthesis engine using minimal counterexamples,
(constant) bounded counterexamples and positive bounded counterexamples 
as $\engine_{\infmncegis}$, $\engine_{\infbcegis}$ and $\engine_{\infhmncegis}$ respectively
where the verifier $\verifier$ is replaced by $\mnverifier$,
$\bverifier$ and $\hmnverifier$ respectively in 
the definition of $\engine_{\infcegis}$. The languages identified by these 
synthesis engines are denoted by $\infmncegis$, $\infbcegis$ and $\infhmncegis$ respectively.

Similarly, $\engine_{\mncegis}$, $\engine_{\bcegis}$ and $\engine_{\hmncegis}$ are 
obtained from  $\engine_{\cegis}$ by replacing the verifier $\verifier$ by $\mnverifier$,
$\bverifier$ and $\hmnverifier$ respectively. The
languages identified by these 
synthesis engines are denoted by $\mncegis$, $\bcegis$ and $\hmncegis$ respectively.


\comment{
\subsection{Background}

 It is also
known that no class of language
with at least one infinite language over the same vocabulary as the rest of the languages in the class, can be learnt purely
from positive examples. We can illustrate this infeasibility of
identifying languages from positive examples with a simple
example.

Consider a vocabulary $V$ and let $V^*$ be all the strings that can be formed using vocabulary $V$. The strings in $V^*$ are $x_1, x_2, \ldots$. Let us consider the set of languages
$$L_1 = V^* - \{x_1\}, L_2 = V^* - \{x_2\}, \ldots$$
Now a simple algorithm to learn languages from positive examples can guess the language to be $L_i$ if $x_i$ is the string with the smallest index not seen so far as a positive example. This algorithm can be used to inductively identify the correct language using
just positive examples. But now, if we add a new language $V^*$ which contains all the strings from vocabulary $V$ to our class of language, that is, $$L_2 = V^*, V^* - \{x_1\}, L_2 = V^* - \{x_2\}, \ldots$$
The above algorithm would fail to identify this class of languages.

In fact, no algorithm using positive examples would be able to inductively identify this 
class of languages!\cite{gold67limit}. 
The key intuition is that if the data is all positive, no finite trace of positive data can distinguish whether the currently guessed language is the target language or is merely a subset of the target language. Now, if we consider the presence of negative counterexamples, the learning or synthesis
algorithm can begin with the first guess as $V^*$. If there are no counterexamples, then $V^*$ is the
correct language. If a counterexample $x_i$ is obtained, then the next guess is $V^* - \{x_i\}$, and
this is definitely the correct language.
}



\comment{ 
\textbf{TODO: fix min-inductive synth and historybounded-inductive synth accordingly}

\textbf{Not fixed notations below}
Now, we consider a variant of counterexample guided inductive synthesis where we use minimal counterexamples instead of arbitrary counterexamples $\mncegis$. 

\begin{definition}
A $\mncegis$ engine $\engine_{\mncegis} : \sigma \times \sigma \rightarrow \mathscr{\algo}$ is defined recursively below.\\
$\engine_{\mncegis} (\trace[n], \ce[n]) = F( \engine_{\mncegis} (\trace[n-1], \ce[n-1]),  \trace(n), \ce(n) ) $\\
where $F$ is a recursive function $\mathscr{\algo} \times \nat \times \nat \rightarrow \mathscr{\algo}$ that characterizes the learning engine and how it eliminates counterexamples, $\trace[n]$ is a trace for language $\lang$ and
$\ce$ is a counterexample sequence such that\\
$\ce(i) = \mnverifier_\lang(\lang(\engine_{\mncegis}(\trace[i-1], \ce[i-1]))) $.\\
$\engine_{\mncegis} (\sigma_0, \sigma_0)$ is a predefined constant representing an initial guess $\algo_0$ of the program, which for example,
could be program corresponding to the language $\nat$.
\end{definition}



The convergence of the $\mncegis$ synthesis engine to a language and family of languages is defined in similar way as $\cegis$.

\begin{definition}
We say that $\engine_{\mncegis}$ converges to $\algo_i$, that is,
$\engine_{\mncegis}(\trace, \ce) \rightarrow \algo_i$
if and only if
there exists $k$ such that for all
$n\geq k$, $\engine_{\mncegis}(\trace[n], \ce[n]) = \algo_i$.
\end{definition}

\begin{definition}
$\engine_{\mncegis}$ identifies a language $\lang_i$ if and only if for all traces
$\trace$ of the language $\lang_i$
and counterexample sequences $\ce$,
$\engine_{\mncegis}(\trace, \ce) \rightarrow \algo_i$.
$\engine_{\mncegis}$ identifies a language family $\mathscr{\lang}$ if and only if $\engine_{\mncegis}$ identifies every $\lang_i \in \mathscr{\lang}$.
\end{definition}



\begin{definition}
$\mncegis = \{ \; \mathcal{L} \; | \; \exists \engine_{\mncegis} \; .\; \engine_{\mncegis}$ identifies $\mathscr{\lang} \}$
\end{definition}

Next, we consider another variant of counterexample guided inductive synthesis $\hmncegis$ where we use {\it history bounded} counterexamples instead of arbitrary counterexamples. We define a history bounded counterexample generating verifier before defining $\hmncegis$. Unlike the previous
cases, the verifier for generating history bounded counterexample is also provided
with the trace seen so far by the synthesis engine. The verifier generates a counterexample
smaller than the largest element in the trace. If there is no counterexample smaller than the
largest element in the trace, then the verifier does not return any counterexample.
From the definition below, it is clear that we need to only order elements in the language
and do not need to define an ordering of $\bot$ with respect to the language
elements since the comparison is done between an element in non-empty $\lang \cap \lang_i$
and elements $\trace[j]$ in the trace.

\begin{definition}
A  {verifier} $\hmnverifier_\lang$ for a language $\lang$ is a mapping from $\mathscr{\lang} \times \sigma $ to $\nat \cup \bot$ such that\\ $\hmnverifier_\lang(\lang_i,\trace[n]) = m$ where $m \in \overline \lang \cap \lang_i \wedge m < \trace(j)$ for some $j \leq n$, and $\hmnverifier_\lang(\lang_i,\trace[n]) = \bot$ otherwise.
\end{definition}


\begin{definition}
A $\hmncegis$ engine $\engine_{\hmncegis} : \sigma \times \sigma \rightarrow \mathscr{\algo}$ is defined recursively below.
$\engine_{\hmncegis} (\trace[n], \ce[n]) = F( \engine_{\hmncegis} (\trace[n-1], \ce[n-1]),  \trace(n), \ce(n) ) $\\
where $F$ is a recursive function $\mathscr{\algo} \times \nat \times \nat \rightarrow \mathscr{\algo}$ that characterizes the learning engine and how it eliminates counterexamples, $\trace[n]$ is a trace for language $\lang$ and
$\ce$ is a counterexample sequence such that\\
$\ce(i) = \hmnverifier_\lang(\lang(\engine_{\mncegis}(\trace[i-1], \ce[i-1])), \trace[i-1]) $.\\
$\engine_{\hmncegis} (\sigma_0, \sigma_0)$ is a predefined constant representing an initial guess $\algo_0$ of the program, which for example,
could be program corresponding to the language $\nat$.
\end{definition}



The convergence of the $\hmncegis$ synthesis engine to a language and family of languages is defined in similar way as $\cegis$ and $\mncegis$.


\begin{definition}
We say that $\engine_{\hmncegis}$ converges to $\algo_i$, that is,
$\engine_{\hmncegis}(\trace, \ce) \rightarrow \algo_i$
if and only if
there exists $k$ such that for all
$n\geq k$, $\engine_{\hmncegis}(\trace[n], \ce[n]) = \algo_i$.
\end{definition}

\begin{definition}
$\engine_{\hmncegis}$ identifies a language $\lang_i$ if and only if for all traces
$\trace$ of the language $\lang_i$
and counterexample sequences $\ce$,
$\engine_{\hmncegis}(\trace, \ce) \rightarrow \algo_i$.
$\engine_{\hmncegis}$ identifies a language family $\mathscr{\lang}$ if and only if $\engine_{\hmncegis}$ identifies every $\lang_i \in \mathscr{\lang}$.
\end{definition}


\begin{definition}
$\hmncegis = \{ \; \mathcal{L} \; | \; \exists \engine_{\hmncegis} \; .\; \engine_{\hmncegis}$ identifies $\mathscr{\lang} \}$
\end{definition}
}


==> ogis-old.tex <==
\section{Oracle-Guided Inductive Synthesis: $\ogis$} \label{sec-ogis}

\comment{
\begin{figure}[htb!]
\centering%
\scalebox{0.7}{\includegraphics{ogis}}
\caption{Oracle Guided Inductive Synthesis}
\label{fig:ogis}
\end{figure}
}

\begin{figure}[htb!]
\centering
\includegraphics[height=5cm]{ogis.pdf}
\caption{Oracle Guided Inductive Synthesis}
\label{fig:ogis}
\end{figure}


We illustrate {\it {Oracle-Guided Inductive Synthesis}} ($\ogis$) paradigm in Figure~\ref{fig:ogis}.
It consists of two key components: Inductive Learning Engine and Oracle. Synthesis is an iterative
process which involves a series of queries from the inductive engine to oracle, and corresponding
responses from the oracle to the induction engine. 
We first discuss these components in general and then present examples to 
illustrate how synthesis techniques
from formal methods and machine learning can be presented as an instantiation of $\ogis$. 
The inductive learning engine has a
learning bias which could restrict the search space of programs to a particular class. This
corresponds to program template such as restrictions to programs
generated using a context-free grammar in SyGus~\cite{alur-fmcad13} synthesis
problems. This is often referred to as concept class in machine learning literature~\cite{angluin88}.
An $\ogis$ algorithm for program
synthesis can specify the inductive learning bias as a program template.
Further, $\ogis$ requires specification of an inductive learning algorithm
which generalizes from examples. 
The algorithm used for induction can be restricted by the computational complexity
as well as by the assumptions on its memory. 
The oracle is privy to some knowledge about the synthesis target as well as the class of programs
under consideration. It could have the complete specification of the program in some logical form
or as an unoptimized programs. It could also be an incomplete specification or just a set of 
input/output examples of the program. The oracle has one or more algorithms to reply to queries 
from the inductive engine. For example, equivalence checking algorithm and the knowledge of the complete
specification can be used to reply to {\it equivalence} queries from the inductive engine. We 
give examples of types of queries and corresponding responses that can take place between 
the inductive learning engine and the oracle.
\begin{enumerate}
\item Membership query: The inductive learning engine can query with an example. The oracle knows
the target concept and can send a response whether the example is in the target language or not.
\item Witness query: The learning engine can query oracle which knows the target concept to provide
an example in the target language.
\item Equivalence query: The learning engine can propose a candidate hypothesis program. The oracle
can compare with its knowledge of correct program and send a response with either just yes/no or 
also provide a counterexample if the hypothesis is wrong. Equivalence query with 
arbitrary counterexamples is used in $\tcegis$ approaches to program synthesis~\cite{asplos06}.
\item Subsumption query: This is similar to equivalence query but it only checks whether
the hypothesis program is contained in the target program or not. This is often easier in
practice.
\item Distinguishing input query: The learning engine can propose a candidate hypothesis program
and the set of examples used to generate the program. The oracle can generate alternate hypothesis
programs from the set of examples and generate examples on which the alternate hypothesis differs
from the candidate hypothesis program sent by the learning engine. This example is then
completed using the knowledge of oracle about the target program and returned to the learning engine.
A practical implementation of this approach for synthesizing programs has been previously
presented~\cite{jha-icse10}.
\end{enumerate}

We now take three example synthesis techniques previously presented in literature and illustrate
how they instantiate the $\ogis$ paradigm.
\begin{example}  Automata synthesis~\cite{Angluin-queries}:\\
The first synthesis technique is the classic work on learning concepts from 
membership and equivalence queries by Angluin~\cite{Angluin-queries}. The inductive bias
in Angluin's concept learning is to assume that the concepts are subsets of a
{\it finite} set of examples. Thus, the concept class is the power set of the set of examples.
For any hypothesis concept which is itself a subset of the examples, Angluin uses membership
and equivalence queries to the oracle. The oracle knows the target language and can provide
counterexamples for equivalence queries. The counterexample is assumed to be generated 
{\it adversarially}. 
\end{example}
\begin{example} Counterexample-guided inductive synthesis~\cite{asplos06}:\\
The second synthesis technique is $\tcegis$~\cite{asplos06} which can be used
to solve a SyGuS synthesis problem~\cite{alur-fmcad13}. The inductive bias is the restriction
that the concept class of programs can be described as a context-free language. $\tcegis$ uses
equivalence/subsumption queries. The oracle has the complete specification of the program and hence,
it can check any candidate program using traditional formal verification techniques~\cite{clark-smt}.
An arbitrary counterexample is returned by the oracle if the candidate hypothesis program was incorrect.
$\tcegis$ also assumes that the set of programs is finite to ensure termination of the synthesis
algorithm.
\end{example} 
\begin{example} Oracle-guided program synthesis using distinguishing inputs~\cite{jha-icse10}:\\
The third synthesis engine is based on using distinguishing inputs when complete specification
is not available~\cite{jha-icse10}. The inductive bias is provided in form of a finite library of
component functions, and the program is restricted to by a composition of a subset of these
components. A distinguishing input query is made to the oracle. The oracle does not know the complete
specification of the program apriori but it can provide output of the program for a given input. The
oracle discovers an input on which the hypothesis program differs from another consistent program 
based on the examples seen so far, and generates the output for this input. This is returned
as a distinguishing example to the inductive engine for further generalization. Similar to above
approaches, it also assumes a finite space to ensure termination of the synthesis algorithm.
\end{example}

In this paper, we consider a general setting where the concept class of programs
is the set of programs corresponding to the set of recursive (decidable languages).
The language is defined over an infinite alphabet and the set of 
recursive languages (and hence, the programs) is also infinite. We choose such an expressive
class of programs because we want to compare the synthesis techniques by varying the oracle,
and the nature of responses from the oracle. We choose subsumption query 
and witness query as the form of communication
between the inductive synthesis engine and the oracle. This is similar to the existing
synthesis techniques. The oracle knows the target concept and it 
can provide witnesses or positive examples to the induction engine
and also provide counterexamples. We consider four different types of counterexamples 
that the oracle can provide. Each of this type describes a different oracle and hence, a different
synthesis technique. Our goal is to compare these synthesis techniques and establish whether
one type of counterexample allows the synthesis technique to successfully learn more programs than 
the other. The four kinds of counterexamples considered in this paper are as follows:
\begin{itemize}
\item First, we consider {\it arbitrary} counterexamples. This is equivalent to the case of $\tcegis$ but
we are applying it to a class of infinite programs and not finite set of programs and examples as in
the previous work~\cite{asplos06}. So, termination is no longer guaranteed. 
This serves as the baseline for comparison against other synthesis techniques.
\item Second, we consider {\it minimal} counterexamples instead of arbitrary counterexamples. For any predefined ordering on the examples, we require that the validation engine provide a counterexample which is minimal. This choice of counterexamples is motivated by literature on debugging. Significant effort has been made on improving validation engines to produce counterexamples which aid debugging by localizing the error~\cite{antonio13,ChenSMV10}. The use of counterexamples in $\tcegis$ conceptually is an iterative repair process and hence, it is natural to extend successful error localization and debugging techniques to inductive synthesis. 
\item Third, we consider {\it bounded} counterexamples where the counterexamples produced by the
validation engine is bounded by a constant. This is motivated by the use of bounds in formal
verification such as bounded model checking~\cite{biere-bmc} and 
verification of concurrent programs~\cite{qadeer-bounded} using bounds on context-switches.
\item Fourth, we consider {\it positive bounded} counterexamples where the counterexample produced by the validation 
engine must be smaller than a previously seen positive example. This is motivated from the 
industrial practice of validation by simulation where the system is often simulated to a finite length to 
discover bugs. The length of simulation often depends on the traces which illustrate known positive behaviors.
It is expected that errors will show up if the system is simulated up to the length of the largest positive trace.
\end{itemize}
We also consider two kinds of inductive generalization algorithms:
\begin{itemize}
\item First, we consider inductive algorithms which do not have any memory bound and the memory can grow 
indefinitely. This is motivated by $\tcegis$ where the set of counterexamples and positive examples are 
collected throughout the algorithm. For the space of infinite programs, this set can grow unbounded and is potentially
infinite.
\item Second, we consider inductive algorithms for which memory is restricted to be finite and hence,
the inductive algorithm is iterative. It takes existing hypothesis and the set of positive examples and
counterexamples to produce a new hypothesis program. Such a restriction on memory is more practical.
\end{itemize}

The synthesis engine using arbitrary counterexamples and with infinite memory is motivated
by $\tcegis$ algorithm~\cite{asplos06} and hence, we refer to it as $\infcegis$ in the paper even though
it was used for finite programs in the previous work. The variant of $\infcegis$ which is restricted to
use finite memory is referred to as $\cegis$. Similarly, the the synthesis engine
using minimal counterexamples and infinite memory is called minimal counterexample guided inductive
synthesis, aka, $\infmncegis$. The variant of the approach using finite memory is referred to as $\mncegis$. 
The synthesis engine using counterexamples which are smaller than the largest positive examples 
is called positive-history bounded counterexample and is referred as $\infhmncegis$ if the memory is not
finite and $\hmncegis$ if the memory is finite. 


%\footnote{ Practically, this would mean replacing satisfiability solving based verification engines with those using Boolean optimization such as maximum satisfiability solving techniques.}
For the class of programs corresponding to the set of recursive languages,
our focus is on decidability, that is, whether the synthesis technique terminates with 
the correct program or not. This question is interesting since our concept class is not finite. 
We do not discuss computational complexity of synthesis, and the impact of different types
of counterexamples on the speed of convergence in this paper. Computational complexity for
infinite class of programs for which synthesis is guaranteed to terminate is left as a topic
for future research.
 
We also consider $\ogis$ techniques which restrict the concept class of programs to be finite.
The decidability question for finite class of programs is trivial since the termination
is guaranteed as long as the queries provide new examples or some new information about the 
target program. But the speed at which the synthesis approach converges remains relevant even 
for finite class of programs. We show
that the computational complexity of these techniques is related to 
Vapnik-Chervonenkis dimensions~\cite{Blumer-vp}.

\comment{
For each of the variants of $\cegis$, we analyze whether it increases
the candidate spaces of programs where a synthesizer terminates with correct program.
We prove the following in the paper.
\begin{enumerate}
\item $\mncegis$ successfully terminates with correct program on a candidate space if and only if
$\cegis$ also successfully terminates with the correct program. So, there is no increase or decrease
in power of synthesis by using minimal counterexamples.
\item $\hmncegis$ can synthesize programs from some program classes where $\cegis$ fails to synthesize
the correct program. But contrariwise, $\hmncegis$ also fails at synthesizing programs from some program
classes where $\cegis$ can successfully synthesize a program. Thus, their synthesis power is not
equivalent, and none dominates the other.
\end{enumerate}

Thus, none of the two counterexamples considered in the paper are strictly {\it good} mistakes.
The history bounded counterexample can enable synthesis in additional classes of programs but
it also leads to loss of some synthesis power.
 



  
Sec. 4: Finite Domains
  - Teaching Dimension: a property of the concept class that gives a lower bound on
    number of iterations of CEGIS, also for learning with distinguishing inputs.
    --> does TD also give a lower bound for ALL OGIS techniques?

Sec. 5: Infinite Domains
   - Specific questions: What is the impact of the following factors on termination of OGIS loop?
      i) Type of counterexamples given by O
     ii) Resources available to L
   - Describe the following four variants of CEGIS:
      a) Arbitrary CEGIS (arbitrary counterexamples)
      b) Min CEGIS (min counterexamples according to some fixed but unspecified cost function)
      c) Constant bounded CEGIS (counterexamples whose "value", according to some computable function,
              is bounded by a constant --- motivate this by all the "bounding" techniques for bug-finding:
              BMC, context-bounding, delay-bounding, etc.)
      d) History bounded CEGIS (counterexamples whose value is bounded by history of previous examples)
           -- Note: rename "trace" to "history" in our previous draft
   - Results:
      * CEGIS = MinCEGIS
      * CB-CEGIS < CEGIS
      * HB-CEGIS != CEGIS (incomparable)
      I suppose we could also show that CB-CEGIS < HB-CEGIS? (encode the constant bound into the synthesis problem?)
    - Discussion: would be good to add some discussion about how these results are relevant to, say, SyGuS for QFLRA

Sec. 6: Conclusion and Open Problems
 - Summarize our results (maybe in a table?)
 - Pose various other questions and open proble

}


==> res-oct2015.tex <==

\section{Theoretical Analysis of CEGIS: Results}
\label{sec-res}
\label{sec:res}
%\section{Infinite Program Classes}~\label{sec-res}

In this section, we present the theoretical results when the class of languages 
(programs) is infinite.
\revise{ We consider two axes of variation. 
We first consider the case in which the inductive learning
technique has finite memory in Section~\ref{sec-resfin}, 
and then the case in which it has
infinite memory in Section~\ref{sec-resinf}.  
For both cases, we consider the four kind of counterexamples mentioned in Section~\ref{sec-intro}
and Section~\ref{sec-not};
namely, arbitrary counterexamples, minimal counterexamples, bounded counterexamples and 
positive bounded counterexamples. }
%compare $\mncegis$ and
%$\cegis$ in the first part of the section followed by $\hmncegis$ and $\cegis$ in the second part of the
%section. Since 
%We focus on analyzing the impact of change in the power of formal synthesis
%techniques which use oracles that provide different kinds of counterexamples.
%So, we fix the inductive learning engine $\learner$,
% and denote it by $F$.
%Thus, we vary the counterexample generating verifier serving as oracle in $\ogis$:
%$\verifier_\lang$, $\mnverifier_\lang$, $\bverifier_\lang$ and
%$\hmnverifier_\lang$, but 
%inductive learning technique is the same $F$ and the \todo{transcript} of 
%positive examples $\trace$ is same. This allows us to study the impact
%of using different verifiers in isolation from the rest of the $\ogis$
%framework.

%In the
%rest of the section, we present the two central results of this paper:
%\begin{enumerate}
%\item $\mncegis = \cegis$
%\item $\hmncegis \not = \cegis$
%\end{enumerate}

\subsection{Finite Memory Inductive Synthesis}
\label{sec-resfin}

We investigate the four language classes $\cegis, \mncegis, \bcegis$ and  $\hmncegis$  identified by
the synthesis engines  $\engine_{\cegis}$, $\engine_{\mncegis}$, $\engine_{\bcegis}$ and $\engine_{\hmncegis}$
and establish relations between them. We show that $\bcegis \subset \mncegis = \cegis$, 
$\hmncegis \not \subseteq \cegis$ and $\hmncegis \not \supseteq \cegis$.


\subsubsection{Minimal vs. Arbitrary Counterexamples}

We begin by showing that replacing a deductive
verification engine which returns arbitrary counterexamples with a deductive verification engine which 
returns minimal counterexamples does not change the power of counterexample-guided inductive synthesis.
\revise{The 
%main result regarding this non-intuitive fact that there is no change in the
%power of synthesis technique by using
%minimal counterexamples 
result is summarized in Theorem~\ref{thm-min}.}

\begin{theorem} \label{thm-min}
The power of synthesis techniques using arbitrary counterexamples and those using minimal counterexamples are 
equivalent, that is, $\mncegis = \cegis$.
\end{theorem}

\begin{proof}
$\mnverifier$ is a special case of $\verifier$ in that a minimal counterexample
reported by $\mnverifier$ can be treated as arbitrary counterexample to simulate $\cegis$ using 
$\mncegis$. 
%Intuitively,
%using minimal counterexample is not worse than using arbitrary counterexamples.
Thus, $\cegis \subseteq \mncegis$.

The more interesting case to prove is $\mncegis \subseteq \cegis$. For a language $\lang$, 
let $\mncegis$ converge to the correct 
%program $\algo$, that is $\langfun(\algo)=\lang$, 
language $\lang$ on  \todo{transcript} $\trace$. 
We show that $\engine_{\cegis}$ can simulate $\engine_{\mncegis}$ and also converge to $\lang$
%$\algo$
on \todo{transcript} $\trace$.
The proof idea is to show that a finite learner can simulate
$\mnverifier$ by making a finite number of calls to $\verifier$. 
Let the arbitrary counterexample returned by verifier
for a candidate language $\lang_i$ at any step of the synthesis
engine be $c$, that is $\verifier(\lang, \lang_i) = c$. 
Then, $\verifier(\lang \cap \{c\}, \lang_i \cap \{c\}) \not = \bot$ 
and hence, $c$ is upper bound on the number of 
times that $\verifier$ needs to be called in finding the minimum 
counterexample. Thus,
$$\mnverifier(\lang, \lang_i) = \text{ minimum } j \text{ such that }  \verifier(\lang \cap \{j\}, \lang_i \cap \{j\}) \text{ is not } \bot \text{ for } 0 \leq j \leq \verifier(\lang, \lang_i) $$
 We only need finite memory to 
store the current value of  $j$ while iteratively calling the verifier 
$\verifier$.  Thus, $\mnverifier(\lang,\lang_i)$ can be computed
using finite memory and using at most $k= \verifier(\lang, \lang_i)$ calls of $\verifier$. So, $\engine_{\cegis}$ can simulate $\engine_{\mncegis}$
by finding the minimal counterexample at each step using the verifier
$\verifier$ iteratively as described above. 

Thus, $\mncegis = \cegis$.
\qed

\end{proof}


\comment{
We  use an auxiliary variable to store a language of the form $\lang_{0i}
= \{ j | j \leq i \text{ and } j \geq 0 \}$ where $i$ is bounded by the largest minimal
counterexample obtained during synthesis by $\engine_{\mncegis}$. 
This language is used in framing the correct
verification query for finding minimal counterexamples. \\
$$\engine_{sim}(L_0, \trace[n]) = \lang_n  \; \mathtt{ where } \; \lang_{i} = \learner (\lang_{i-1}, \trace(i), \mncemap(\lang_{i-1})) \; \mathtt{for} \; i=1,2,\ldots,n $$

Given a candidate language $\lang_i$, we can find the minimal counterexample
for $\lang_i$ using only an arbitrary counterexample generation verifier
$\verifier$ using the following technique. 
The proof idea is to simulate $\engine_{\mncegis}$ in two phases. In one phase, $\engine_{\cegis}$ finds the 
minimal counterexample~\footnote{The elements in our language are natural numbers with
a total ordering and hence, we can ensure that the counterexample is minimum.
In general, the ordering could be partial and the counterexample
is only minimal.} for a candidate language $L_j$ by iteratively calling $\verifier$. In the second phase, $\engine_{\cegis}$ 
consumes the next elements from the \todo{transcript}. 
While searching for minimal counterexample, $\engine_{\cegis}$ needs 
to store the backlog of the \todo{transcripts}. 

We describe a simulation of $\engine_{\mncegis}$ using $\verifier$. 
The simulation uses two auxiliary variables: one to store the 

We define a mapping $\engine_{sim}$ from $\mathscr{\lang} \times \Sigma \rightarrow \mathscr{\lang}$ which simulates $\engine_{\mncegis}$ while maintaining the backlog. Since the learner
has finite memory, we will also show that the backlog is always finite. 
We also use an auxiliary variable to store a language of the form $\lang_{0i}
= \{ j | j \leq i \text{ and } j \geq 0 \}$ where $i$ is bounded by the largest minimal
counterexample obtained during synthesis by $\engine_{\mncegis}$. 
This language is used in framing the correct
verification query for finding minimal counterexamples. \\
$$\engine_{sim}(L_0, \trace[n]) = \lang_n  \; \mathtt{ where } \; \lang_{i} = \learner (\lang_{i-1}, \trace(i), \mncemap(\lang_{i-1})) \; \mathtt{for} \; i=1,2,\ldots,n $$
We need to prove that $\mncemap$ can be computed with finite bounded memory
and finite bounded time in order to establish that $T_{sim}$ can 
simulate $\engine_{\mncegis}$ with finite memory. 
$$\mncemap(\lang_i) = \text{ minimum } i \text{ such that }  \verifier(\lang \cap \lang_{0i}, \lang_i \cap \lang_{0i}) \text{ is not empty }$$
Starting from $\lang_{00}$ and enumerating $\lang_{01}, \lang_{02} \ldots$, the computation of $\mncemap$ would find the 
minimum $i$ such that the verification query returns a counterexample if 
$\lang_i$ is not the correct language. This counterexample is clearly the
minimum counterexample. The number of queries needed is bounded by the 
size of the largest minimum counterexample in $\engine_{\mncemap}$. 
While the minimum counterexample is being bound, the incoming transcript
is stored in the backlog for being processed later. The size of this backlog
is bounded by the length of the transcript used by $\engine_{\mncemap}$ to
converge the correct language multiplied by the size of the largest
minimum counterexample used by $\engine_{\mncemap}$. Thus, 
$\engine_{\sim}$ can simulate $\engine_{\mncemap}$ using finite bounded
memory.
}

\comment{
$\mncemap$ denotes a mapping from languages to minimal counterexamples if 
one exists and is known during simulation. 
$$\mncemap: \mathscr{\lang} \rightarrow \nat \cup \{ \top \} \cup \{ \bot \}$$
Intuitively, this maps a candidate language $\lang_i$ 
 to  minimal counterexample as known 
to $\engine_{\cegis}$ so far in simulating $\engine_{\mncegis}$. $\mncemap$ maps the languages for which minimal counterexamples
are unknown to $\top$. If there is no counterexample to a given language, 
$\mncemap$ maps the language to $\bot$. At any given step, only finite number of languages have their minimal 
counterexamples known, and the rest are mapped to $\top$.\\
\\
We define a mapping $\engine_{\mncemap}$ from 
$\mathscr{\lang} \times \Sigma \rightarrow \mathscr{\lang}$ which simulates
$\engine_{\mncegis}$ based on the known $\mncemap$ so far, that is,
$$\engine_{\mncemap}(\lang_0, \trace[n]) = \lang_n \; \mathtt{ where } \; \lang_{i} = \learner (\lang_{i-1}, \trace(i), \mncemap(\lang_{i-1})) \; \mathtt{for} \; i=1,2,\ldots,n \; \mathtt{and} \; \lang_0 = lang$$
if $\mncemap(\lang_{i})$ is not $\top$ for $i=1,2,\ldots$ and it is undefined if  $\mncemap(\lang_{i})$ is 
$\top$ for any $i$. 

We now present the formal description of the proof.
For this simulation, we use some auxiliary variables maintained by 
$\engine_{\cegis}$ which store some finite information required
for simulating $\engine_{\mncegis}$. The key idea is for $\engine_{\cegis}$ to iteratively guess the minimal 
counterexample in multiple micro-steps
and then use that to simulate one step of $\engine_{\mncegis}$. 
%But simulating each step of $\engine_{\mncegis}$ takes finite number
%of micro-steps for $\engine_{\cegis}$ and uses finite storage.\\
\\
The first auxiliary component for this simulation is a minimal counterexample map
\comment{Intuitively, this maps a candidate program $\algo_i$ (language $\lang_i$) to  minimal counterexample as known 
to $\engine_{\cegis}$ so far in simulating $\engine_{\mncegis}$. If minimal counterexample is not known for a 
given program, $\mncemap$ maps the program to $\top$. If there is no counterexample to a given program, 
$\mncemap$ maps the program to $\bot$. At any given step, only finite number of programs have their minimal 
counterexamples known, and the rest are mapped to $\top$.}

Next, \\The first auxiliary component for this simulation is a minimal counterexample map
$$\mncemap: \mathscr{\lang} \rightarrow \nat \cup \{ \top \} \cup \{ \bot \}$$

Next, we define a mapping $\engine_{\mncemap}$ from 
$\mathscr{\lang} \times \Sigma \rightarrow \mathscr{\lang}$ which simulates
$\engine_{\mncegis}$ based on the known $\mncemap$ so far, that is,
$$\engine_{\mncemap}(\lang_0, \trace[n]) = \lang_n \; \mathtt{ where } \; \lang_{i} = \learner (\lang_{i-1}, \trace(i), \mncemap(\lang_{i-1})) \; \mathtt{for} \; i=1,2,\ldots,n \; \mathtt{and} \; \lang_0 = \lang$$
if $\mncemap(\lang_{i})$ is not $\top$ for $i=1,2,\ldots$ and it is undefined if  $\mncemap(\lang_{i})$ is 
$\top$ for any $i$. \\
\\
$\engine_{\mncemap}$ simulates $\engine_{\mncegis}$ using the same counterexamples and intermediate candidate languages 
for the known positive history $\mncemap$. If $\mncemap$ is $\top$ for any of the intermediate languages, $\engine_{\mncegis}$
is undefined.
Further, we record the language proposed by $\engine_{\mncegis}$ into the variable $\lang_\siml^m$ and the last
 language which initiated search for minimal counter example in $\lang_{last}$. 
\todo{A candidate language belongs to the indexed
family of languages and hence,
it is represented by its index.
The intermediate hypothesis languages occupy unit memory and this 
 enables us to record a bounded number of 
 intermediate hypothesis languages. 
 Such a memory model is used in learning theory
 literature to analyze whether a language family is learnable
 by recording only a finite number of intermediate hypothesis
 and a finite number of examples~\cite{gold67limit,jain1999systems} }.
$\trace_\siml^m$  records
the part of the \todo{transcript} already simulated by $\engine_{\cegis}$ and $\mu$ is the candidate minimal counterexample
while searching for minimal counterexample.
The maximum length of $\trace_\siml^m$ and 
the number of languages $\lang$ in $\mncemap$ not mapped
 to $\top$ is bounded by the length of the
 \todo{transcript} 
 required to converge to correct language by $\engine_{\mncegis}$
 that we are simulating. Hence, the memory required to store
 these auxiliary variables is also bounded. 
\\
\\
\noindent \textbf{Initialization}:
All the internal auxiliary variables are initialized as follows. $\lang_\siml^0 = \lang_0$ which is the same initialization as
$\engine_{\mncegis}$ being simulated, $\mu = 0$, $\lang_{last} = \lang_0$, and $\trace_\siml^0 = \sigma_0$. $\mncemap$ is initialized
to map all $\lang$ to $\top$ as no minimal counterexamples are known at the beginning.\\
\\
\noindent \textbf{Update}:
We describe the updates made in each iteration $m$. One of the following cases is true in each iteration.\\
\textbf{Case 1}: If $\lang_{last} = \lang_\siml^m$,  that is, we are in lock-step with the $\mncegis$ synthesis algorithm with the same candidate language.\\
\textbf{Case 1.1}: If there is any counterexample for $\lang_\siml^m$ (found using the verifier for $\engine_{\cegis}$), that is, the candidate
language has a counterexample and we need to find the corresponding minimal counterexample.\\
\textbf{Case 1.1.1}: If $\mncemap(\lang_\siml^m)$ is not $\top$, that is, the minimal counterexample for candidate language is already part of
$\mncemap$.\\
Let $\trace_{done}$ be the longest prefix for $\trace_\siml^m \trace(m+1)$ such that $\engine_{\mncemap}(\lang_\siml^m, \trace_{done})$ is defined. Since $\mncemap(\lang_\siml^m)$ is not $\top$, $\trace_{done}$ is not empty.
$\trace_{done} \trace_\siml^{m+1} = \trace_\siml^m \trace(m+1)$, $\lang_\siml^{m+1} = \engine_{\mncemap}(\lang_\siml^m, \trace_{done})$, $\lang_{last} = \lang_\siml^{m+1}$\\
We use the minimal counterexample from $\mncemap$ and then advance the simulation $\trace_{done}$ \todo{transcript}  
ahead if $\engine_{\mncemap}$ can simulate
the \todo{transcript} 
using minimal counterexamples from $\mncemap$  for all the intermediate candidate languages.\\
\textbf{Case 1.1.2}: If $\mncemap(\lang_\siml^m)$ is $\top$, that is, the minimal counterexample for candidate language is not known.\\
 $\trace_\siml^{m+1} = \trace_\siml^m \trace(m+1)$, $\lang_\siml^{m+1} = \lang_\siml^m \cap \{0\}$.\\
We initialize the candidate language $\lang_\siml^{m+1} $ for searching for minimal counterexample to  
$\lang_\siml^{m} \cap \{0\}$, that is,
it is either the language consisting only of the minimal element $\{ 0\}$ or is empty depending
on whether the minimal element belongs to the target language or not.
Since our verifier uses a subset query, empty language will return no counterexamples.  \\
\textbf{Case 1.2}: If there is no counterexample for $\lang_\siml^m$,\\
Let $\trace_{done}$ be the longest prefix for $\trace_\siml^m \trace(m+1)$ such that $\engine_{\mncemap}(\lang_\siml^m, \trace_{done})$ is defined.
$\trace_{done} \trace_\siml^{m+1} = \trace_\siml^m \trace(m+1)$, $\lang_\siml^{m+1} = \engine_{\mncemap}(\algo_\siml^m, \trace_{done})$, $\lang_{last} = \lang_\siml^{m+1}$
and $\mncemap(\lang_\siml^m) = \bot$.\\
The candidate language seen so far is subset of the target language and we consume as much of the \todo{transcript} $\trace_{done}$  as possible
for which $\engine_{\mncemap}$ is defined. \\
\\
\textbf{Case 2}: If $\lang_{last} \not = \lang_\siml^m$, that is, the simulation is trying to find the minimal counterexample as a result of case 1.1.2.\\
\textbf{Case 2.1}: If there is any counterexample $\ce_\siml$ for $\lang_\siml^m$ (found using the verifier for $\engine_{\cegis}$),\\
 Update $\mncemap(\lang_{last}) = \ce_\siml$. Let $\trace_{done}$ be the longest prefix for
$\trace_\siml^m \trace(m+1)$ such that $\engine_{\mncemap}(\lang_{last}, \trace_{done})$ is defined.
$\trace_{done} \trace_\siml^{m+1} = \trace_\siml^m \trace(m+1)$, $\lang_\siml^{m+1} = \engine_{\mncemap}(\lang_{last}, \trace_{done})$, $\lang_{last} = \lang_\siml^{m+1}$, $\mu = 0$\\
If there is a counterexample, since the candidate language was a single element set or empty, and verification engine checks for
containment in the target language, the only element in the language has to be the counterexample. 
\todo{Further, 
%starting from step 1.1.2 and with
%possible increments in step 2.2, 
this is the minimal counterexample (minimality is due to step
1.1.2 and step 2.2), 
and we add it to the $\mncemap$.}\\
\textbf{Case 2.2}: If there is no counterexample for $\lang_\siml^m$, that is, we have not yet found the minimal counterexample.\\
$\mu = \mu +1 $, $\lang_\siml^{m+1} = \lang_{last} \cap \{\mu\}$, and  $\trace_\siml^{m+1} = \trace_\siml^m \trace(m+1)$.\\
We increment $\mu$ and search for whether $\lang_{last} \cap \{\mu\}$ is in the target language. This is either empty or is a language
consisting of a single element $\{\mu\}$.\\
\\
\textbf{Progress}:
Now, we first show progress of the simulation in parsing \todo{transcript} $\trace[m]$. For any $m$, there exists $m' > m$ such that $\trace[m] = \trace_{done}^m \trace_\siml^m$, $\trace[m'] = \trace_{done}^{m'} \trace_\siml^{m'}$ and $\trace_{done}^{m}$ is a proper prefix of
$\trace_{done}^{m'}$. This follows from the observation that Case 2.2 cannot be repeated infinitely after Case 1.1.2 since $\lang_{last}$ has at least one counterexample. So, case 2.1 would eventually become true and hence, 
$\mncemap$ is extended. So, $\engine_{\mncegis}$ would be defined for a longer prefix and case 1.1.1
would be true. And consequently, the \todo{transcript} $\trace_{done}$ simulated so far is extended. \\
\\
\textbf{Correctness}:
Let $\engine_{\mncegis}$ converge on $\trace$ after reading prefix $\trace[n]$. 
From progress, after some $m \geq n$, $\trace[n]$ would
be a prefix of $\trace_{done}^m$. Since $\engine_{\mncegis}$  converges after reading 
$\trace[n]$, $\learner(\lang_n,\trace(n'),\ce(n')) = \lang_n$
for $n' > n$. Now, $\mncemap$ is not $\top$ for all intermediate languages 
$\lang_{m''}$ in $\engine_{\mncegis}$ for $m'' \leq m$.
So, $\lang_\siml^{m} = \engine_{\mncemap}(\lang_\siml^0, \trace[m]) = \engine_{\mncemap}(\lang_0, \trace[m]) = \lang_n$ and
for all $m' > m \geq n$, $\lang_\siml^{m'} = \learner(\lang_n,\trace(n),\ce(n))  = \lang_n$
So, $\engine_{\cegis}$ also converges to
$\lang_n$, that is, $\mncegis \subseteq \cegis$.\\
\\
}

Thus, $\mncegis$ successfully converges to the correct language 
 if and only if
$\cegis$ also successfully converges to the correct language. So, there is no increase or decrease
in power of synthesis by using deductive verifier that provides minimal counterexamples.

%\subsection{Synthesis Using {\it \bf History Bounded} Counterexamples}

\subsubsection{Bounded vs. Arbitrary Counterexamples}

We next investigate $\bcegis$ and compare its relative synthesis power compared to $\cegis$.
As intuitively expected, $\bcegis$ is strictly less powerful than $\cegis$ as summarized
in Theorem~\ref{thm-b} which formalizes the intuition. 

\begin{theorem}
The power of synthesis techniques using bounded counterexamples 
is less than those using counterexamples, that is, $\bcegis \subset \cegis$.
\label{thm-b}
\end{theorem}

\begin{proof}
Since bounded counterexample is also a counterexample, we can easily simulate a bounded verifier
$\bverifier$ using a $\verifier$ by ignoring counterexamples from $\verifier$ if they are larger
than a specified bound $\bound$ which is a fixed parameter and can be stored in the finite memory
of the inductive learner. Thus, $\bcegis \subseteq \cegis$. 

We now describe a language class  for which the corresponding languages
cannot be identified using bounded counterexamples.
\begin{langfamily}
: $\mathcal{\lang}_{notcb} =\{ \lang_i |  
\todo{\lang_i \subseteq \{ n | n \in \nat \wedge n > \bound \}}
\}$ where
$\bound$ is the bound used by the verifier producing constant bounded counterexamples.
\label{lf:cbweak}
\end{langfamily}
The language family~\ref{lf:cbweak} formed by lower bounding the elements by some fixed constant, that is,
\todo{$\lang_i \subseteq \{ n | n \in \nat \wedge n > \bound \}$} where $\bound$ is the bound used
by the verifier producing bounded counterexamples. 
Clearly, such a verifier would not return 
any counterexample for a language in this class and hence, $\engine_\bcegis$ cannot identify languages in this class of languages while $\engine_\cegis$ can. So, $\bcegis \subset \cegis$.

\qed
 
\end{proof}


We next analyze $\hmncegis$,  and show that it is not equivalent to $\cegis$ or contained in it.
So, replacing a deductive verification engine
which returns arbitrary counterexamples with a verification engine which returns
counterexamples bounded by history of positive examples has impact on the power of the synthesis technique.
But this does not strictly increase the power of synthesis. Instead, the
use of positive history bounded counterexamples allows languages from
new classes to be identified but at the same time, language from some
language classes which could be identified by 
$\cegis$ can no longer be identified using positive bounded counterexamples.
The main result regarding the power of synthesis techniques using
 positive bounded counterexamples is summarized in Theorem~\ref{thm-hb}.

\begin{theorem} \label{thm-hb}
The power of synthesis techniques using arbitrary counterexamples and those using
positive bounded counterexamples are not equivalent, and none is more powerful than the other.
$\hmncegis \not = \cegis$. In fact,  $\hmncegis \not \subseteq \cegis$ and $\cegis \not \subseteq \hmncegis$.
\end{theorem}

We prove this using the following two lemma. The first lemma \ref{lemma-cegisbetter}
shows that there is a family of
languages from which a language can be identified by $\cegis$ but,
this cannot be done by $\hmncegis$. The second lemma \ref{lemma-hcegisbetter} shows that
there is another family of languages from which a language can be identified by
$\hmncegis$ but not by $\cegis$.


\begin{lemma} \label{lemma-cegisbetter}
There is a family of languages $\mathcal{L}$ such that 
$\hmncegis$ cannot identify a language 
$\lang$ in $\mathcal{L}$ but
$\cegis$ can identify  $\lang$, that is,
 $\cegis \not \subseteq \hmncegis$
\end{lemma}

\begin{proof}
Now, consider the language family~\ref{lf:pbweak} formed by upper bounding the elements by some fixed constant. Let the target language $\lang$ (for which we want to identify $\lang_i$. In rest of the proof, we also refer to this family as $\mathcal{L}$ for brevity.
\begin{langfamily}
$\mathcal{L}_{notpb} = \{ \lang_i | i \in \nat \}$ such that 
$$\lang_i = \{ n | n \in \nat \wedge n \leq i \}$$
\label{lf:pbweak}
\end{langfamily}


If we obtain a \todo{transcript} $\trace[j]$ at any point in synthesis
using positive bounded counterexamples, then for any intermediate language $\lang_j$ proposed by
$\engine_{\hmncegis}$, $\hmnverifier_\lang$  would always return $\bot$ since all the counterexamples
would be larger than any element in $\trace[j]$. This is the consequence of the chosen languages
in which all counterexamples to the language are larger than any positive example of the language.
So, $\engine_{\hmncegis}$ cannot identify the target language $\lang$.

But we can easily design a synthesis engine $\engine_{\cegis}$
using arbitrary counterexamples that can synthesize
$\algo$ corresponding to the target language $\lang$. The algorithm starts with $L_0$ as its
initial guess. If there is no counterexample, the algorithm next guess is $\lang_1$.
In each iteration $j$,
the algorithm guesses $\lang_{j+1}$ as long as there are no counterexamples. When a counterexample
is returned by $\verifier_\lang$ on the guess $\lang_{j+1}$,
the algorithm stops and reports the previous guess $\lang_j$ as the correct language.

Since the elements in each language $\lang_i$ is bounded by some fixed constant $i$, the above synthesis procedure $\engine_{\cegis}$ is guaranteed to terminate after $i$ iterations when identifying any language $\lang_i \in \mathcal{L}$. Further, $\verifier_\lang$ did not return any counterexample up to iteration $j-1$ and so, $\lang_j \subseteq \lang_i$. And in the next iteration, a counterexample was generated.
So, $\lang_{j+1} \not \subseteq \lang_i$. Since, the languages in $\mathcal{L}$ form a monotonic chain
$\lang_0 \subset \lang_1 \ldots $. So, $\lang_j = \lang_i$. In fact, $j=i$ and in the $i$-th iteration,
the language $L_i$ is correctly identified by $\engine_{\cegis}$.

Thus,  $\cegis \not \subseteq \hmncegis$.


\qed

\end{proof}

This shows that $\cegis$ can be used to identify languages when $\hmncegis$ will fail. Putting a
restriction on the verifier to only produce counterexamples which are bounded by the
positive examples seen so far does not strictly increase the power of synthesis.

We now show that this restriction enables identification 
of languages which cannot be identified by $\cegis$. 
%The proof uses a
%diaganolization argument similar to the argument used in \cite{Lange08} for showing the
%increase in inductive synthesis power when negative examples are introduced in addition
%to the positive examples.
%Recall that the set of languages considered in that case were
%$L_1 = V^* - \{x_1\}, L_2 = V^* - \{x_2\}, \ldots$ and the language $V^*$. The argument
%relies on indistinguishability of  $V^* - \{x_1\}$ and  $V^*$ with respect to finite traces
%of positive examples.

In the proof below, we construct a language which is not distinguishable
using arbitrary counterexamples and instead, it relies on the verifier keeping a record of the
largest positive example seen so far and restricting counterexamples to those below the largest positive
example. 


\begin{lemma} \label{lemma-hcegisbetter}
There is a family of languages $\mathcal{L}$ such that, $\cegis$ cannot identify a  language $\lang$ in $\mathcal{L}$ but
$\hmncegis$ can identify  $\lang$, that is,
 $\hmncegis \not \subseteq \cegis$
\end{lemma}


\begin{proof}
Consider the language 
$$\lang^{32} = \{ 3^j.2^i | j \in \{0,1\}, i \in \nat \}  $$ 
We now construct a family of languages which are finite subsets of $\lang^{32}$ and have 
at least one member of the form $3.2^i$, that is,
$$\mathcal{L}^{32} = \{\lang^{32}_i | i \in \nat, \lang^{32}_i \subset \lang^{32}, \lang^{32}_i \text{ is finite } \text{ and } \exists k \; s.t. 
\; 3.2^k  \in \lang^{32}_i \}$$
We now consider the language
$$\lang^2 = \{ 2^i | i \in \nat\}$$ 
Now, let $\mathcal{\lang}^{2}$ be the family of languages such that the smallest element member in the language 
is the same as the index of the language, that is,
$$\mathcal{\lang}^{2} = \{ \lang^2_i | i \in \nat,  \lang^2_i \subseteq \lang^2, \lang^2_i \text{ is infinite and } \min(\lang^2_i) = 2^i \}$$

Now, we consider the following family of languages below.
\begin{langfamily} $$ \mathcal{L}_{pb} = \mathcal{L}^{32} \cup \mathcal{L}^{2}$$
\label{lf:pb} 
\end{langfamily}
We refer to this language as $\mathcal{L}$ in rest of the proof for brevity.
We show that there is a language $\lang$ in $\mathcal{L}$ such that the 
language 
$\lang$ cannot be identified by $\cegis$ but $\hmncegis$ can 
identify 
any language in $\mathcal{L}$.

The key intuition is as follows.
If the examples seen by synthesis algorithm till some iteration $i$ are all of the form 
$2^j$, then any synthesis technique cannot differentiate whether the
language belongs to $\mathcal{L}^{32}$ or $\mathcal{L}^{2}$. If the language belongs
to  $\mathcal{L}^{32}$, the synthesis engine would eventually obtain
an example of the form  $3.2^j$ (since each language in $\mathcal{L}^{32}$
has at least one element of this kind and these languages are finite). While
the synthesis technique using arbitrary counterexamples cannot recover the previous examples,
the techniques with access to the verifier which produces positive bounded counterexamples
can recover all the previous examples.

We now specify a $\engine_\hmncegis$ which can identify languages in $\mathcal{L}$. The synthesis approach works in two possible steps.
\begin{itemize}[leftmargin=*]
\item Until an example $3.2^j$ is seen by the synthesis engine, let $2^i$ be the smallest member element
seen so far in the \todo{transcript}, the learner proposes $\lang_i$ as the language. If the target
language $\lang \in \mathcal{L}^{2}$, the learner would eventually identify the language since
the minimal element will show up in the  \todo{transcript}.
If the target language $\lang \in \mathcal{L}^{32}$, then eventually, an example of the form
$3.2^j$  will be seen since $\lang$ must have one such member element. And after such an example 
is seen in the \todo{transcript}, the synthesis engine moves to second step.
\item After an example of the form $3.2^j$ is seen, the synthesis engine can now be sure that the language
belongs to $\mathcal{L}^{32}$ and is finite. Now, the learner can discover all the positive examples 
seen so far
using the following trick. We first discover the upper bound $B_p$
on positive examples seen so far.
$$B_p = \text{ minimum k such that } \hmnverifier(\{3^k\}, \lang \cap \{3^k\}, \trace[n]) \text{ returns }  \bot \text{ for } k = 2,3,\ldots$$  
Recall that $3^k, k = 2,3, \ldots$ are not in the target language
since they are not in any of the languages in the $\mathcal{L}$ to which the target language belongs.
$\hmnverifier$ will return the only element $3^k$ in the proposed
candidate language as a counterexample as long as
there is some positive example $2^i$ seen previously such that $2^i \geq  3^k$. So, $3^{B_p}$ is the upper bound on all the positive examples seen
 so far.
The learner can now construct singleton languages 
$\{2^j\}$ for $j=0,1,... l$ such that $2^l < 3^{B_p}$. 
If a counterexample is returned 
by $\hmnverifier(\{2^i\}, \lang \cap \{2^i\}, \trace[n])$ 
then $2^i$ is not in the target language.
If no counterexample is returned, then $2^i$ is in the target language. This allows the synthesis engine
to recover all the positive examples seen previously in finite steps.
% and a hypothesis language is constructed 
%by adding all of these. And all the positive examples seen henceforth are added to the hypothesis language.
As we recover the positive examples, we run a Gold style
algorithm for identifying finite languages~\cite{jain07} 
to converge to the correct language.
%Since the language is finite, this will consume finite memory and terminate after finite steps. 
Thus, the learner would identify the correct language using finite memory.   
\end{itemize}
 
 
We now prove the infeasibility of $\cegis$ for this class of languages. Let us
assume that $\mathcal{L} \in \cegis$. So, there is a synthesis engine $\engine_\cegis$
which can identify languages in $\mathcal{L}$. So, $\engine_\cegis$ must converge to any language $\lang_1 \in \mathscr{L}^2$ after some finite
transcript $\tau_s$. Let us consider an extension $\tau_s 2^m$ of $\tau_s$ 
such that $2^m \in \lang_1$ and $2^m \not \in \samples(\tau_s)$. Such 
an element $2^m$ exists 
since $\tau_s$ is a finite transcript and $\lang_1$ is an
infinite language. Since the learner converges to $\lang_1$
starting from the initial language $\lang_0$ 
after consuming $\tau_s$, $\learner(\lang_0,\tau_s2^m, \ce') = \learner(\lang_0, \tau_s, \ce)$.

Let us consider two transcripts $\tau_s 2^m (3.2^p)^\omega$ and 
$\tau_s (3.2^p)^\omega$ where $(3.2^p)^\omega$ denotes repeating
$3.2^p$ infinitely in the rest of the transcript.
We know that $\learner(\lang_0,\tau_s 2^m, \ce') = \learner(\lang_0, \tau_s, \ce) = \lang_1$
and thus, $\learner(\tau_s 2^m (3.2^p)^\omega, \ce') =  \learner(\tau_s (3.2^p)^\omega, \ce) = \learner(\lang_1, (3.2^p)^\omega, \ce'') $. So, the synthesis engine would behave exactly for both
transcripts, and if it converges to a language $\lang_2$ on one transcript, it would converge to the same language on the other transcript. But the two
transcripts are clearly from two different languages in $\mathcal{L}^{32}$.
One of the transcripts corresponds to
the finite language $\samples(\trace_s) \cup \{3.2^p\}$
and the other corresponds to $\samples(\trace_s) \cup \{2^m,3.2^p\}$.
This is a contradiction and hence, there is no synthesis engine using
arbitrary counterexamples
$\engine_{\cegis}$ that can identify all languages in $\mathcal{L}$. 

\qed


\comment{
\begin{algorithm}                      % enter the algorithm environment
\caption{Construction of the diagonal language $\lang_d$}          % give the algorithm a caption
\label{alg-hbproof}                           % and a label for \ref{} commands later in the document
%\begin{algorithmic}[H]
$s = 0$, $Done = false$\\
\While{$!Done$} {
    $Done = true$\\
   \If {there exists a $\tau \subseteq \tau_s$ s.t. $\lang_s = \engine_{\hmncemap}(\lang_0, \trace[n]) \not \in \negset $, $\lang_s \cap \overline {\samples(\tau_s)}$ is not empty and $\tau$ is shortest such \todo{transcript}} 
       {
          \tcc{*********Diagonalization*********}
          Let $x \in \lang_s \cap \overline { \samples(\tau_s) } $\\ 
          Extend the negative set of examples: $\nex := \nex \cup \{x\}$;\\
          Extend the counterexample map: $\cemap(\lang_s) = x$;\\
          $\tau_{s+1} = \tau_s$;
          $s = s+1$;
          $Done = false$\\
       }
   \If{there exists a $\tau \supseteq \tau_s$ such that $samples(\tau) \subseteq \{ 2^i | i \geq m \} \setminus \nex$, $\engine_{\hmncemap}(\lang_0, \trace[i])$ is defined for all $i \leq |\tau|$ and $\engine_{\hmncemap}(\lang_0, \trace) \not = \engine_{\hmncemap}(\lang_0, \trace_s)$}
      {
        \tcc{*********Add to language $\lang_d$*********}
        $\tau_{s+1} = \tau$;
        $\lang_d := \lang_d \cup \{ 2^i | 2^i \in \samples(\tau) \}$;
        $s = s + 1$;
        $Done = false$\\
      }
}
%\end{algorithmic}
\end{algorithm}



We construct a diagonal language $\lang_d$ using the simulation of the synthesis engine $\engine_\cegis$.
Initially, we have $\lang_m = \{2^m\}$ for some $m \in \nat$ such that $\lang_m$ is the initial guess of the
synthesis engine.
We construct two auxilary storage to contain the simulation information: 
\begin{itemize}
\item $\nex$ is the set of negative examples outside the language being constructed. We initialize $\nex$
to $\{3^i.2^j | i > 1 \} \cup \{ 2^i | i <  m \} $. It is augmented by all counterexamples added during 
the simulation of the synthesis engine.
\item The second is a counterexample map
$$\cemap: \mathscr{\lang} \rightarrow \nex \cup \{ \top \} \cup \{ \bot \}$$
Intuitively, this maps a candidate language $\lang_i$ to  a counterexample as known 
to $\engine_{\hmncegis}$ so far. When a counterexample is known, it is added to the
$\nex$ set. If a counterexample is not known for a 
given language, $\cemap$ maps the language to $\top$. If there is no counterexample to a given language, 
$\cemap$ maps the language to $\bot$. At any given step, only finite number of languages have their  
counterexamples known, and the rest are mapped to $\top$.
\end{itemize}  


Next, we define a mapping $\engine_{\hmncemap}$ from 
$\mathscr{\lang} \times \Sigma \rightarrow \mathscr{\lang}$
based on the known $\cemap$ so far, that is,
$$\engine_{\hmncemap}(\lang_0, \trace[n]) = \lang_n \; \mathtt{ where } \; \lang_{i} = \learner (\lang_{i-1}, \trace(i), \cemap(\lang_{i-1})) \; \mathtt{for} \; i=1,2,\ldots,n \; \mathtt{and} \; \lang_0 = \lang$$
if $\cemap(\lang_{i})$ is not $\top$ for $i=1,2,\ldots$ and it is undefined if  $\cemap(\lang_{i})$ is 
$\top$ for any $i$. \\ 
%$\cexmap$ is a map from hypothesis programs to counterexamples. Initially, it is empty
We denote the set of hypothesis languages already proven to be incorrect (since they produce a counterexample)
by $\negset = \{ \lang_i | \cemap(\lang_i) \in \nex \}$ 


Let $\trace_s$ denote the \todo{transcript} simulated so far upto some step $s$. $\trace_0$ is a single member \todo{transcript} 
containing $2^m$. 
The construction of diagonal language is shown in Algorithm~\ref{alg-hbproof}. 
We first assume that the loop terminates for some $s$. So, $\lang_d = \samples(\trace_s) = \langfun(\lang_s)$.
So, for all intermediate hypothesis languages proposed by the algorithm at step $s'$, we have
$\langfun(\lang_{s'}) \subseteq \langfun(\lang_s)$ or  $\langfun(\lang_{s'}) \in \negset$.
Now, we consider two languages corresponding to the contents of two \todo{transcripts}: $\tau_s \; 2^p \; 3.2^q$ and
 $\tau_s \; 3.2^q$ where $p \geq m $ and $2^p \not \in \nex$ and $\nex$ is the set of counterexamples obtained
for $\tau_s \; 3.2^q$ (such a finite set exists since the synthesis engine must converge on this \todo{transcript}). 
Further, since the second {\it {if}} condition is not true, so for any extension of $\trace_s$ with 
$2^p$ such that , $\engine_{\hmncemap}(\lang_0, \trace_s) = \engine_{\hmncemap}(\lang_0, \trace_s 2^p)$.
So, the counterexample set $\nex$ is the same in simulation of $\engine_{\hmncemap}$ for $\trace_s$ as well as $\trace_s 2^p$. 
The counterexample received after seeing $3.2^q$ is the same for both \todo{transcripts}. So, we observe that the synthesis engine
has the same counterexample set $\nex$ and  $\engine_{\hmncemap}(\lang_0, \trace_s) = \engine_{\hmncemap}(\lang_0, \trace_s 2^p)$.
Thus, the behavior of the engine  $\engine_{\hmncemap}$ is, the same for 
both \todo{transcripts}. So, it cannot identify one of the two languages. This is a contradiction since we assumed that
the synthesis engine can identify any language in the language family $\mathscr{\lang}$. 
Intuitively, the finite memory synthesis engine cannot store all positive examples and we exploit this to show
that after some steps $s$ it cannot distinguish between two languages in $\mathscr{\lang}^{32}$.

So, our assumption that loop terminates for some $s$ is not true. We now consider that the loop does not terminate.
Let us consider the 
\todo{transcript} $\tau = \bigcup_{s\in \nat} \tau_s$, that is the 
concatenation of \todo{transcript} at each step of the simulation.
Now, $\tau$ is a \todo{transcript} for the language $\lang_d$ and $\samples(\tau) = \lang_d$.
If $\engine_{\hmncemap}$ converges for all \todo{transcripts} for all languages in $\mathscr{\lang}$, then it also must converge
on $\lang_d$ for $\tau$. So, after some step $s$, any intermediate conjecture language which enumerates a member element
not in $\samples(\tau) = \lang_d$ is in the $\negset$. Further, if the synthesis engine converges after some step $s$, then
$\engine_{\hmncemap}(\lang_0, \trace[s]) = \engine_{\hmncemap}(\lang_0, \trace[s'])$ for all $s'$. Thus, both the {\it {if} } conditions
are eventually not true and hence, the loop will terminate. This is a contradiction again. And so, no such $\engine_{\hmncemap}$ exists.
\qed
}


\end{proof}

\subsubsection{Different Flavors of Bounded Counterexamples}

Finally, we compare $\hmncegis$ and $\bcegis$ and show that they are not contained in each other.

\begin{theorem}
The power of synthesis techniques using bounded counterexamples 
is neither less nor more than the techniques using positive bounded counterexamples, 
that is, $\bcegis \not \subseteq \hmncegis$ and  $\hmncegis \not \subseteq \bcegis$.
\label{thm-bhb}
\end{theorem}

\begin{proof}
We consider two languages considered in previous proofs and show that the
languages corresponding to one of them
can only be identified by $\hmncegis$ while the 
languages corresponding to the other
can only be synthesized by $\bcegis$.

Consider the language family~\ref{lf:cbweak} ($\mathcal{L}_{notcb}$)
 formed by lower bounding the elements by some fixed constant, that is,
$$\lang_i = \{ n | n \in \nat \wedge n > \bound \}$$ where $\bound$ is the bound used
by the verifier producing bounded counterexamples. Clearly, such a verifier would not return 
any counterexample for a language in this class and hence, $\bcegis$ cannot  identify languages in this class of languages while $\cegis$ can.
Since any counterexample is smaller than all positive examples, a verifier
producing positive bounded counterexample behaves similar to an arbitrary counterexample verifier
and thus, it can identify languages in this language class.
 So, $\hmncegis \not \subseteq \bcegis$.


Consider the languages in the language family
formed by upper bounding the elements by some fixed constant, that is,
$$\lang_i = \{ n | n \in \nat \wedge n \leq i \}$$
Now, consider the family of languages consisting of these, that is,
\begin{langfamily}
$\mathcal{L}_{cbnotpb} = \{ \lang_i | i < \bound \}$ where $\lang_i = \{ n | n \in \nat \wedge n \leq i \}$
\label{lf:cbnotpb}
\end{langfamily}
This is a slight variant of the language class considered in proving $\engine_\cegis$
to be more powerful than $\engine_\hmncegis$ where we have restricted the class of languages
to be a finite set. As stated earlier, $\hmnverifier$ does not produce 
any counterexample for these languages since all positive examples are smaller than
any counterexample. But $\bverifier$ can be used to identify 
languages in this class by selecting the bound to be $\bound$. Since, the counterexamples
are at most of size $\bound$ for these languages, a bounded counterexample verifier 
behaves exactly like an arbitrary counterexample producing verifier.
Thus, $\bcegis \not \subseteq \hmncegis$.
\qed
\end{proof}

\comment{
Let us consider trace $\trace$ and counterexample sequence $\ce$ such that $\engine_\cegis$
converges in $n$ steps, that is $\engine_\cegis(\trace, \ce) \rightarrow \engine_\cegis(\trace[n], \ce[n])$.
Now, $\ce[n]$ is a valid counterexample sequence of any language $L$ such that
$\samples(\trace[n]) \subseteq L \subseteq \nat - \samples(\ce[n])$.
Since $\engine_\cegis$ must
recognize a language from any trace and any arbitrary counterexample sequence, we choose
a trace and counterexample sequence as follows.
Let us consider a trace $\trace'$  of the form $\trace[n] (\langle 1, z_1 \rangle)^\infty$.
The corresponding counterexample trace discovered by $\engine_\cegis$ is $\ce[n]$ followed
by minimal counterexamples, if any, after observing $\langle 1, z_1 \rangle$.
Now, we pick an element
$\langle 0, z_2 \rangle$ such that  $\langle 0, z_2 \rangle \not \in \ce[n]$
and $\langle 0, z_2 \rangle \not \in \trace[n]$.
Since $\ce[n]$ is a valid counterexample sequence of any language $L$ such that
$\samples(\trace[n]) \subseteq L \subseteq \nat - \samples(\ce[n])$, the behavior
of $\engine_\cegis$ is same for $\trace[n] (\langle 1, z_1 \rangle)^\infty$
as it is for $\trace[n] \langle 0, z_2 \rangle (\langle 1, z_1 \rangle)^\infty$.
Thus, $\engine_\cegis$ cannot distinguish between the
two languages: $\lang^d = \samples(\trace[n]) \cup \{ \langle 1, z_1 \rangle) \}$
and  $\lang^{d'} = \samples(\trace[n]) \cup \{ \langle 0, z_2 \rangle, \langle 1, z_1 \rangle) \}$.
Intuitively, $\engine_\cegis$ can forget some positive examples seen before observing  $\langle 1, z_1 \rangle$
and there is no way to regenerate these as it can be done with $\engine_\hmncegis$.


Thus, $\hmncegis \not \subseteq \cegis$.
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Infinite Memory Inductive Synthesis}
\label{sec-resinf}

We now consider the case where inductive learning engine has infinite unbounded memory. This case
is simpler than the one considered earlier with finite memory bound on the inductive learning engine
and most of the results presented here follow from the results proved for the finite memory case.
We make the following observations:
\begin{enumerate}
\item The proof of Theorem~\ref{thm-min} works even when we replace the inductive learning engine
using finite memory with the one using infinite memory. The simulation of $\mnverifier$ by $\verifier$
can be made simpler if the memory is infinite but the simulation used in Theorem~\ref{thm-min} 
also works for the infinite memory case. Further, the minimal counterexample can still be
used as an aribitrary counterexample. And so, $\infmncegis = \infcegis$.
\item Given a bound $\bound$ on the counterexamples produced by $\bverifier$, $\engine_\infcegis$ can 
simulate the synthesis engine $\engine_\infbcegis$ by checking whether the counterexample
from $\verifier$ is smaller than the bound $\bound$. If the counterexample is larger than $\bound$,
then, we remove it from the proposed language and iteratively invoke the verifier $\verifier$ till
we find a counterexample smaller than $\bound$ or we find that no such counterexample exists.
While the check is being done, the positive example \todo{transcript} can be stored using the infinite unbounded
memory.
Thus, $\engine_\infcegis$ can simulate $\engine_\infbcegis$ and so $\infbcegis \subseteq \infcegis$.
\item If the memory of inductive learning engine is not finite, it can store all the examples
that are sent to it. So, the engine $\engine_\infcegis$ can use a verification oracle $\verifier$ providing
arbitrary counterexamples but internally it can compute the positive bounded counterexample
using the recorded history of positive examples. This can be done by checking whether the counterexample
is smaller than at least one of the positive examples seen so far. If it is not so, the counterexample
is removed from the proposed language, and the verification oracle is again queried to obtain a new
counterexample. This terminates when we obtain a counterexample smaller than the largest positive example
seen so far or we discover that no such counterexample exists. 
While the check is being done, the positive example \todo{transcript} can be stored using the infinite unbounded
memory. Thus, $\engine_\infcegis$ can simulate 
$\engine_\infhmncegis$ and hence, $\infhmncegis \subseteq \infcegis$.

\end{enumerate}

We now present three languages used previously in proofs for inductive learning engines using 
infinite memory, and show how these languages allow us to distinguish relative power of synthesis engines.
\begin{enumerate}

\item Consider the language family~\ref{lf:cbweak}: $\mathcal{L}_{notcb} = \{ \lang_i | i \in \nat \}$ where
$$\lang_i = \{ n | n \in \nat \wedge n > \bound \}$$ where $\bound$ is the bound used
by the verifier producing bounded counterexamples. As argued in proof of
Theorem~\ref{thm-b}, such a verifier would not return 
any counterexample for a language in this class and hence, $\engine_\infbcegis$ cannot 
identify languages in this class of languages while $\engine_\infcegis$ can. 
So, $\mathcal{L}_{notcb} \in \overline \infbcegis \cap \infcegis$. 

Further, a positive history bounded verifier will always return a counterexample if one exists
since all counterexamples are larger than any positive example in the language. This, $\engine_\infhmncegis$
can also identify languages in $\mathcal{L}_{notcb}$. 
Thus, $\mathcal{L}_{notcb} \in \overline \infbcegis \cap \infhmncegis$.

\item Consider the language family~\ref{lf:pbweak}: $\mathcal{L}_{notpb} = \{ \lang_i | i \in \nat \}$ where
$$\lang_i = \{ n | n \in \nat \wedge n \leq i \}$$
%Given this family $\mathcal{L}$, let the target language $\lang$ for which we want to synthesize a recognizing program $\algo$ be $\lang_i$. 
As argued in proof of Theorem~\ref{thm-hb}, the verifier 
producing positive bounded counterexamples will not report any counterexample for any of the languages
in $\mathcal{L}_{notpb}$ because all counterexamples are larger than any positive example. So,
 languages in this family cannot be identified by $\engine_\infhmncegis$ but 
these can be identified using $\engine_\infcegis$.
So, $\mathcal{L}_{notpb} \in \overline \infhmncegis \cap \infcegis$. 


\item Consider the finite language family~\ref{lf:cbnotpb}: $\mathcal{L}_{cbnotpb} = \{ \lang_i | i < \bound \}$ where
$$\lang_i = \{ n | n \in \nat \wedge n \leq i \}$$
As argued in proof of Theorem~\ref{thm-bhb}, the verifier  $\hmnverifier$ does not produce 
any counterexample for these languages since all positive examples are smaller than
any counterexample. But $\bverifier$ can be used to identify
languages in this class by selecting the bound to be $\bound$. Since, the counterexamples
are at most of size $\bound$ for these languages, a bounded counterexample verifier 
behaves exactly like an arbitrary counterexample producing verifier.
Thus,  $\mathcal{L}_{cbnotpb} \in \overline \infhmncegis \cap \infbcegis$. 
\end{enumerate}


We now summarize the results described in this section below.
For finite memory learners,
$\bcegis \subset \mncegis = \cegis$, 
$\hmncegis$ and $\cegis$ are not comparabale, that is,
$\hmncegis \not \subseteq \cegis$ and $\hmncegis \not \supseteq \cegis$.
$\bcegis$ and $\hmncegis$ are also not comparable.
In case of infinite memory learners,
$\infbcegis \subset \infmncegis = \infcegis$, and  
$\infhmncegis \subset \infcegis = \infmncegis$.
$\infbcegis$ and $\infhmncegis$ are again not comparable.
The results are summarized in Figure~\ref{fig:summary}.


\begin{figure}[htb!]
\centering
\includegraphics[height=7cm]{summary.pdf}
\caption{Summary of Results on Decidability of Synthesis for Infinite Language Classes}
\label{fig:summary}
\end{figure}

